Graph Partitioning With Limited Moves

In many real world networks, there already exists a (not necessarily optimal) $k$-partitioning of the network. Oftentimes, one aims to find a $k$-partitioning with a smaller cut value for such networks by moving only a few nodes across partitions. The number of nodes that can be moved across partitions is often a constraint forced by budgetary limitations. Motivated by such real-world applications, we introduce and study the $r$-move $k$-partitioning~problem, a natural variant of the Multiway cut problem. Given a graph, a set of $k$ terminals and an initial partitioning of the graph, the $r$-move $k$-partitioning~problem aims to find a $k$-partitioning with the minimum-weighted cut among all the $k$-partitionings that can be obtained by moving at most $r$ non-terminal nodes to partitions different from their initial ones. Our main result is a polynomial time $3(r+1)$ approximation algorithm for this problem. We further show that this problem is $W[1]$-hard, and give an FPTAS for when $r$ is a small constant.

==> checklist.tex <==
\section{CHECKLIST}
\begin{enumerate}


 \item For all models and algorithms presented, check if you include:
 \begin{enumerate}
   \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. [Yes]
   \item An analysis of the properties and complexity (time, space, sample size) of any algorithm. [Yes]
   \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. [No, we will do this upon the acceptance of our paper]
 \end{enumerate}


 \item For any theoretical claim, check if you include:
 \begin{enumerate}
   \item Statements of the full set of assumptions of all theoretical results. [Yes]
   \item Complete proofs of all theoretical results. [Yes, some are in the supplementary materials]
   \item Clear explanations of any assumptions. [Yes]     
 \end{enumerate}


 \item For all figures and tables that present empirical results, check if you include:
 \begin{enumerate}
   \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). [Yes]
   \item All the training details (e.g., data splits, hyperparameters, how they were chosen). [Not Applicable]
         \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). [Not Applicable]
         \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider). [Not Applicable]
 \end{enumerate}

 \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
 \begin{enumerate}
   \item Citations of the creator If your work uses existing assets. [Not Applicable]
   \item The license information of the assets, if applicable. [Not Applicable]
   \item New assets either in the supplemental material or as a URL, if applicable. [Not Applicable]
   \item Information about consent from data providers/curators. [Not Applicable]
   \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. [Not Applicable]
 \end{enumerate}

 \item If you used crowdsourcing or conducted research with human subjects, check if you include:
 \begin{enumerate}
   \item The full text of instructions given to participants and screenshots. [Not Applicable]
   \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. [Not Applicable]
   \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. [Not Applicable]
 \end{enumerate}

 \end{enumerate}


==> ksquaredalg.tex <==
\subsection{$O(kr^2)$-approximation algorithm for Max-$r$-move $k$-partitioning}
In this section we prove Theorem \ref{thm:m2approx}, restated below.

\msquared*

We first prove two essential lemmas.

Let $G$ be an instance of the \maxmove problem, and let $\bar{X}$ be an optimal solution to LP~\ref{tab:maxmove-lp}. Let $G'$ be a subgraph of $G$ with the same vertices as $G$, and $uv\in E(G')$ if $d_{\bar{X}}(u,v)<g$ for a given parameter $g$.
\begin{lemma}\label{lem:connected-comp}
If $g\le\frac{1}{8r}$ then for any two vertices $u,v$ such that $\ell_u\neq \ell_v$ and $X_v^{\ell_v},X_u^{\ell_u}\ge3/4$ we must have that $u$ and $v$ are in different connected components of $G'$. 
\end{lemma}
\begin{proof}
Let $u$ and $v$ be two nodes such that $\ell_u\neq \ell_v$ and ${\bar{X}}_v^{\ell_v},{\bar{X}}_u^{\ell_u}\ge3/4$. Let $A$ be the set of nodes $w\in G$ such that ${\bar{X}}_w^{\ell_w}\ge 3/4$. So $u,v\in A$. By Lemma \ref{lem:size} we have that $|G\setminus A|<4r$. Suppose $u$ and $v$ are in the same connected component. Then there is a path $P$ in $G'$ between $u$ and $v$. WLOG we can assume that $u$ and $v$ are the only nodes in $P$ that are in $A$. This is because if there is $w\in A\cap P$, then either $\ell_w\neq \ell_u$ or $\ell_w\neq \ell_v$ and we consider $uw$ sub-path or $vw$ sub-path of $P$, and continue this until there is no node of $A$ in the path except for the endpoints.

Now by definition of $G'$, for every two consecutive vertices $z,z'$ on the path $P$ we have $d_{\bar{X}}(z,z')< g$. Since obeys the triangle inequality, we have $d_{\bar{X}}(u,v)< 4rg<1/2$ since $|G\setminus A|<4r$. Now observe that ${\bar{X}}_v^{\ell_u},{\bar{X}}_u^{\ell_v}\le 1/4$, so we have $d_{\bar{X}}(u,v)\ge \frac{1}{2}(|{\bar{X}}_v^{\ell_u}-{\bar{X}}_u^{\ell_u}|+|{\bar{X}}_v^{\ell_v}-{\bar{X}}_u^{\ell_v}|)\ge 1/2$, which is a contradiction. %So for all $u,v\in H$ we must have $\ell_u=\ell_v$. Let $i^*$ be $\ell_u$ for all $u\in H$. 
\end{proof}

%Let $A$ be the set of nodes in $G$ with $X_v^{\ell_v}\ge 3/4$. By Lemma \ref{lem:connected-comp}, for every connected component $H$ of $G'$, there is an index $i_H$ such that for all nodes $v\in H\cap A$ we have $\ell_v=i_H$. Let $C_i$ be the set of connected components $H$ where $|H|>6r$ and $i_H=i$. Let $V(C_i)=\cup_{H\in C_i}V(H)$. So intuitively most vertices in $v\in V(C_i)$ we have $\ell_v=i$. Next lemma says that the number of vertices $V(C_i)$ that don't have $\ell_v$ equal to $i$ is very low. Formally if $V_i$ is all the nodes $v$ in $G$ such that $\ell_v=i$, we prove in the next lemma that $|V(C_i)\setminus V_i|$ is small. 

For every connected component $H$ of $G'$ let $r_H:=\sum_{v\in V(H)} (1-{\bar{X}}_v^{\ell_v})$. We show in each component $H$, all except almost $r_H$ nodes are from the same initial partition $i_H$.

\begin{lemma}\label{lem:M2approx-cases}
Suppose $g\le\frac{1}{10kr(r+2)}$. If $r\ge 1$, then for each $H$, there is some partition $i_H$ such that the number of nodes $v$ in $H$ with $\ell_v\neq i_H$ is at most $r_H+\frac{r_H}{r+1}$. %\mina{in the middle of changing something. }
\end{lemma}
\begin{proof}
For every $j\in \{1,\ldots,k\}$ let $V_j$ be all the nodes in $G$ with $\ell_v=j$.
We consider two cases, the first case is when $H$ is small, i.e. $|H|\le 6r$. The second case is when $H$ is large.

\paragraph{Case 1: $H\le 6r$.} 
% First suppose that there is $i$ such that $|V_i\cap H|\ge\ceil{r_H+\frac{r_H}{r+1}}$, and $|H\setminus V_i|\ge \ceil{r_H+\frac{r_H}{r+1}}$. In this case we claim that $i_H=i$. To see this, let $v_0=\arg \min_{v\in V_i\cap V(H)} X_v^{i}$ and let $\alpha=X_{v_0}^{i}$.  
% Let $B_1$ be the $\ceil{r_H+\frac{r_H}{r+1}}$ closest nodes in $H\cap V_i$ to $v_0$. Since there are at most $6r$ nodes in $H$, we have that for any $v\in B_1$, the distance between $v$ and $v_0$ is at most $6r-1$. This means that $|X_v^{i}-X_{v_0}^{i}|\le d_X(v_0,v)< 6rg$ and so $X_v^{i}=X_v^{\ell_v}< \alpha+6rg$. So we have $\sum_{v\in B_1} (1-X_v^{\ell_v})>
% (1-\alpha-6rg)(r_H+\frac{r_H}{r+1})$. 

% Let $B_2$ be a subset of $V(H)\setminus V_i$ of size at least $\ceil{r_H+\frac{r_H}{r+1}}$. For every $v\in V(H)\setminus V_i$, there is a node $u\in V_i\cap H$ such that $v$ is at most $6r$ away from $v$ since $H$ is connected and has at most $6r$ nodes. So we have $|X_v^{i}-X_u^{i}|\le d_X(u,v)< 6rg$ and thus $X_v^{i^*}> X_u^{i}-6rg\ge \alpha-6rg$. Since $\ell_v\neq i$, we have $\sum_{v\in B_2} (1-X_v^{\ell_v}) \ge\sum_{v\in B_2} X_v^{i}> (\alpha-6rg)(r_H+\frac{r_H}{r+1})$. So $\sum_{v\in B_1\cup B_2} (1-X_v^{\ell_v}) > (\frac{r_H}{r+1}+r_H)(1-12rg)=r_H$, where the last equality comes from substituting the value of $g$. This is in contradiction with the definition of $r_H$ and so we must have that $|V(H)\setminus V_i|\le r_H+\frac{r_H}{r+1}$.

Suppose that for every $i\in\{1,\ldots,k\}$, we have that $|V(H)\setminus V_i|> r_H+\frac{r_H}{r+1}$. Consider an arbitrary node $v_0\in V(H)$. Define $\alpha_i:={\bar{X}}_{v_0}^i$ for every $i\in \{1,\ldots,k\}$. Since there are at most $6r$ nodes in $H$, for every node $v$ we have that $v$ is at most $6r-1$ edges away from $v_0$ in $G'$. So $d_{\bar{X}}(v,v_0)<6rg$. Since by Lemma \ref{lem:helper2} for every $i$, $d_{\bar{X}}(v,v_0)\ge |{\bar{X}}_v^i-{\bar{X}}_{v_0}^i|$, we have that ${\bar{X}}_v^i>\alpha_i-6rg$ for every $v\in V(H)$ and every $i$. So we have:

\begin{align*}
    \sum_{v\in H} (1-{\bar{X}}_{v}^{\ell_v}) &= \sum_{v\in H} \sum_{i\neq \ell_v} ({\bar{X}}_v^i) =\sum_{i=1}^{k} \sum_{v, \ell_v\neq i} {\bar{X}}_v^i > \sum_{i=1}^{k} \sum_{v, \ell_v\neq i} \alpha_i-6rg \\
    &> \sum_{i=1}^{k} (r_H+\frac{r_H}{r+1})  (\alpha_i-6rg)=(r_H+\frac{r_H}{r+1})(1-6rkg)>r_H.
\end{align*}
Note that we used the fact that $\sum_i \alpha_i=1$, and in the last inequality we substituted the value of $g$. Since $r_H=\sum_{v\in H} (1-{\bar{X}}_{v}^{\ell_v})$ the above inequality is a contradiction and so there is some $i$ such that $|V(H)\setminus V_i|\le r_H+\frac{r_H}{r+1}$.




\paragraph{Case 2: $|H|> 6r$.} Let $A$ be the set of nodes $v$ such that $\bar{X}_v^{\ell_v}\ge 3/4$. By Lemma \ref{lem:connected-comp}, there is an index $i$ such that for all nodes $v$ in $V(H)\cap A$ we have $\ell_v=i$. We first make a few observations about $i$.
We have that $V(H)\cap A\subseteq V_i$, and thus $|V(H)\setminus V_i|\le |V(H)\setminus A|$. Since by Lemma \ref{lem:size} $|V(H)\setminus A|\le |G\setminus A|< 4r$, we have that $|V(H)\setminus V_i|< 4r$. Moreover we have that $|V(H)\cap V_i|= |H|-|V(H)\setminus V_i|>2r\ge r_H+\frac{r_H}{r+1}$.

We show that $i_H=i$. We need to show that $|V(H)\setminus V_i|\le r_H+\frac{r_H}{r+1}$. For sake of contradiction, suppose that $|V(H)\setminus V_i|> r_H+\frac{r_H}{r+1}$. 


%Observe that for each $H\in C_i$, we have $|H|>6r$. Moreover, $A\cap H \subseteq V_i$ and thus $A\cap H=V_i\cap H$. Since by Lemma \ref{lem:size} $|H\setminus A|\le |G\setminus A|<4r$, we have that $|V_i\cap H |=|A\cap H |=|H|-|H\setminus A|\ge 2r\ge 2r_i$ and $|H\setminus V_i|\le |H\setminus A|<4r$. %Since the weight of each node in the graph is at least one, $|H\setminus A_{i^*}|<4M$.

Let $v_0=\arg \min_{v\in V_i\cap V(H)} \bar{X}_v^{i}$ and let $\alpha=X_{v_0}^{i}$.  
Let $B_1$ be the $\ceil{r_H+\frac{r_H}{r+1}}$ closest nodes in $V(H)\cap V_i$ to $v_0$. Note that $|V(H)\cap V_i|>r_H+\frac{r_H}{r+1}$ so $B_1$ exists. Since there are less than $4r$ nodes in $V(H)\setminus V_i$, we have that for any $v\in B_1$, the distance between $v$ and $v_0$ is at most $4r+|B_1|\le 5r+1\le6r$. This means that by lemma \ref{lem:helper2} and triangle inequality $|{\bar{X}}_v^{i}-{\bar{X}}_{v_0}^{i}|\le d_{\bar{X}}(v_0,v)< 6rg$ and so $\bar{X}_v^{i}={\bar{X}}_v^{\ell_v}< \alpha+6rg$. So we have $\sum_{v\in B_1} (1-{\bar{X}}_v^{\ell_v})>
(1-\alpha-6rg)(r_H+\frac{r_H}{r+1})$. 

Let $B_2$ be a subset of $V(H)\setminus V_i$ of size at least $\ceil{r_H+\frac{r_H}{r+1}}$. For every $v\in V(H)\setminus V_i$, there is a node $u\in V_i\cap V(H)$ such that $v$ is at most $4r$ away from $u$ since $H$ is connected and $|V(H)\setminus V_i|<4r$. So by lemma \ref{lem:helper2} and triangle inequality we have $|{\bar{X}}_v^{i}-{\bar{X}}_u^{i}|\le d_X(u,v)< 4rg$ and thus ${\bar{X}}_v^{i}> {\bar{X}}_u^{i}-4rg\ge \alpha-4rg$. Since $\ell_v\neq i$, we have $\sum_{v\in B_2} (1-{\bar{X}}_v^{\ell_v}) \ge\sum_{v\in B_2} {\bar{X}}_v^{i}> (\alpha-4rg)(r_H+\frac{r_H}{r+1})$. So $\sum_{v\in B_1\cup B_2} (1-{\bar{X}}_v^{\ell_v}) > (\frac{r_H}{r+1}+r_H)(1-10rg)>r_H$, where the last inequality comes from substituting the value of $g$. This is in contradiction with the definition of $r_H$ and so we must have that $|V(H)\setminus V_i|\le r_H+\frac{r_H}{r+1}$.
\end{proof}


Next we are going to put these two lemmas together to make a simple algorithm.
%\mina{$g^*$ is the integrality gap}


%\arash{ Now, I believe it. But, still don't think we need 10K in the factor. }

\begin{proofof}{Theorem \ref{thm:m2approx}}
Our algorithm is depicted in Algorithm \ref{alg:M2approx}.
\begin{algorithm}[h]
\caption{$O(kr^2)$-Approximation algorithm for \maxmove}\label{alg:M2approx}
\begin{algorithmic}[1]
   \State $\bar{X}\gets$ solution to the LP of Table \ref{tab:maxmove-lp}. 
    \State $A\gets$ any $v\in V(G)$ with $\bar{X}_v^{\ell_v}\ge 3/4$.
    %\State $A'\gets V(G)\setminus A$
    \State Create the graph $G'$: $V(G'):=V(G)$ and $uv\in E(G')$ if $uv\in E(G)$ and $d_X(u,v)<g=\frac{1}{10r(r+2)k}$.
    \For{Every connected component $H$ of $G'$}
        %\State $r_H\gets \sum_{v\in H} (1-X_v^{\ell_v})$.
        \State $i^*_H\gets\arg \max_{j=1}^k |\{v\in V(H)|\ell_v=j\}|$.
        \State Assign all the nodes in $H$ to $i^*_H$.
    \EndFor
\end{algorithmic}
\end{algorithm}
It first considers an optimal solution $\bar{X}$ of LP~\ref{tab:maxmove-lp}. %Let $A$ be the set of nodes $v$ such that $X_v^{\ell_v}\ge 3/4$. Let $A'$ be the rest of the nodes. By Lemma \ref{lem:size}, we have that $|A'|< 4M$. %Otherwise $\sum_{u\in H'} X_u^{\ell_u}< 3|H'|/4\le |H'|-M$, and so $\sum_{v\in V(G)} X_v^{\ell_v}\le n-M$. 
Then the algorithm generates a new graph $G'$ with vertices of $G$ as follows. Let $g=\frac{1}{10M(M+1)(k+1)}$. For every $u$ and $v$, attach $u$ and $v$ in $G'$ if they are attached in $G$ and $d_{X}(u,v):=\frac{1}{2}\sum_i |X_u^i-X_v^i|< g$. %Moreover, if $u,v\in H$, then attach $u$ to $v$.  
%Let $\bar{Z}$ be the optimal integer solution to the \maxmove instance. 

%\mina{If $|H'|\le M$, just put them wherever you want.}

Then the algorithm takes each connected component $H$ of $G'$ and assigns all of its nodes to one partition $i$. This partition is the partition that the majority of the nodes in $H$ belong to in the initial partitioning, i.e. $i^*_H=\arg \max_{j=1}^k |\{v\in V(H)|\ell_v=j\}|$. 

Now we prove that the cut value of the solution of the algorithm is at most $\frac{1}{g}OPT$ and the algorithm moves at most $r$ nodes.

Proving the approximation guarantee is simple. Denote the solution of the algorithm by $Z$. So if node $u$ is assigned to partition $j$ in the algorithm, we have $Z_u=e_i$. Note that each connected component is in one partition so for each edge $uv$ in the cut set we have that $u$ and $v$ belong to different connected components of $G'$. So $d_{\bar{X}}(u,v)\ge g$. So $1=d_Z(u,v)\le \frac{1}{g}d_{\bar{X}}(u,v)$. Let the set of edges of $G$ that are between the connected components of $G'$ be $E'$. Thus we have
\begin{align*}
    \sum_{uv\in E(G)} c_{uv}d_Z(u,v) &= \sum_{uv\in E'} c_{uv}d_Z(u,v) 
    \le \frac{1}{g}\sum_{uv\in E'} c_{uv}d_{\bar{X}}(u,v)\\
    &\le \frac{1}{g}\sum_{uv\in E(G)} c_{uv}d_{\bar{X}}(u,v)=\frac{1}{g}OPT
\end{align*}
Next we prove that the algorithm moves at most $r$ nodes from their initial partition. For each $j\in \{1,\ldots,k\}$, let $V_j$ be the nodes $v$ in $G$ that are initially in partition $j$, i.e. $\ell_v = j$.

By Lemma \ref{lem:M2approx-cases}, for each connected component $H$, there is $i_H$ such that $|V(H)\setminus V_{i_H}|\le r_H+\frac{r_H}{r+1}$. If $i^*_H=\arg \max_{j=1}^k |\{v\in V(H)|\ell_v=j\}|$, then we have $|V(H)\cap V_{i^*_H}|\ge |V(H)\cap V_{i_H}|$. So $|V(H)\setminus V_{i_H^*}|\le |V(H)\setminus V_{i_H}|$ and thus $|V(H)\setminus V_{i_H^*}|\le r_H+\frac{r_H}{r+1}$. So from component $H$, the algorithm has moved at most $r_H+\frac{r_H}{r+1}$ nodes. So in total, the algorithm has moved at most $\sum_{H} r_H+\frac{r_H}{r+1} \le r+\frac{r}{r+1}$. Since the number of nodes moved is an integer, the algorithm has moved at most $\floor{r+\frac{r}{r+1}}=r$ nodes.

For the running time, solving the LP takes $T(n)$ time. Computing $G'$ and the rest of the algorithm takes $O(mk)$ time.
\end{proofof}





==> leo_experiments.tex <==

\subsection{Experiments on Synthetic Networks}
In our next set of experiments, we evaluate the performance of the FPTAS on synthetic data and use the greedy algorithm as a benchmark to asses the efficacy of the FPTAS. We first discuss the set-up and then the observed results for these experiments.

\begin{figure}
\centering
\begin{subfigure}
  \centering
  % include first image
  \includegraphics[width=.7\textwidth]{prob_1-1.jpg}  
  \caption{Performance of the greedy algorithm and the FPTAS (Algorithm~\ref{alg:fptas}) for different values of $\alpha$ with respect to the solution of LP \ref{tab:maxmove-lp} for the explained stochastic block graphs with $p_L=0.1$ and $p_H=0.1$.}
  \label{fig:FPTAS_1}
\end{subfigure}
\begin{subfigure}
  \centering
  % include second image
  \includegraphics[width=.7\textwidth]{prob_2-1.jpg}  
  \caption{Performance of the greedy algorithm and the FPTAS (Algorithm~\ref{alg:fptas}) for different values of $\alpha$ with respect to the solution of LP \ref{tab:maxmove-lp} for the explained stochastic block graphs with $p_L=0.1$ and $p_H=0.2$.}
  \label{fig:FPTAS_2}
\end{subfigure}
\begin{subfigure}
  \centering
  % include third image
  \includegraphics[width=.7\textwidth]{prob_3-1.jpg}  
  \caption{Performance of the greedy algorithm and the FPTAS (Algorithm~\ref{alg:fptas}) for different values of $\alpha$ with respect to the solution of LP \ref{tab:maxmove-lp} for the explained stochastic block graphs with $p_L=0.1$ and $p_H=0.3$.}
  \label{fig:FPTAS_3}
\end{subfigure}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{prob_4-1.jpg}
    \caption{Performance of the greedy algorithm and the FPTAS (Algorithm~\ref{alg:fptas}) for different values of $\alpha$ with respect to the solution of LP \ref{tab:maxmove-lp} for the explained stochastic block graphs with $p_L=0.1$ and $p_H=0.4$.}
    \label{fig:FPTAS_4}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{prob_5-1.jpg}
    \caption{Performance of the greedy algorithm and the FPTAS (Algorithm~\ref{alg:fptas}) for different values of $\alpha$ with respect to the solution of LP \ref{tab:maxmove-lp} for the explained stochastic block graphs with $p_L=0.1$ and $p_H=0.5$.}
    \label{fig:FPTAS_5}
\end{figure}

\paragraph{Set-up:} We create our sample graphs by employing the stochastic block model on a set of $20$ nodes using the following procedure. For further information on the stochastic block model please refer to section~\ref{sec:exp}. Initially, the $20$ nodes are evenly divided into three clusters of equal size. Subsequently, an edge is added between any two nodes within the same cluster with a probability of $p_H$, and between any two nodes in different clusters with a probability of $p_L$, where we set $p_L$ to 0.1. Various values of $p_H$ from the set $\{0.1, 0.2, 0.3, 0.4, 0.5\}$ are tested. This partitioning closely resembles the optimal $k$-partitioning for $k=3$. Therefore, we randomly re-partition the constructed graph into three partitions. These newly randomized partitions are established as the initial partitioning of the graph. Following these procedures, a total of 50 such random graphs are generated. 

\paragraph{Results:} We experiment with different values of $\alpha\in\{1.1,1.3,1.5,1.7\}$ for the FPTAS algorithm to analyze its performance and dependency on $\alpha$. For each of the 50 random graphs and each of the two algorithms (greedy and Algorithm~\ref{alg:fptas}), we calculate the following ratios: The algorithm's output divided by the objective value of LP \ref{tab:maxmove-lp}. For each $r$ value in $\{1,2,3,4,5\}$, we compute the average of this ratio across all graphs. Refer to Figures~\ref{fig:FPTAS_1}-\ref{fig:FPTAS_5} for the performance of these algorithms for different values of $p_H$. Similar to our experiments with real-world data, we observe that for smaller $r$ values, the greedy algorithm tends to perform reasonably well. In fact, for $r=1$, it often outperforms the FPTAS, specifically for $\alpha=1.3, 1.5, 1.7$. However, as $r$ increases, the greedy algorithm's performance degrades, while the FPTAS's performance improves, regardless of the chosen value of $\alpha$. This behavior is due to the fact that the greedy algorithm makes myopic decisions about moving nodes between partitions, while the FPTAS selects the best solution from the set of nodes it considers for movement. Furthermore,  regardless of the value of $r$, the FPTAS with $\alpha=1.1$ yields solutions very close to those of LP \ref{tab:maxmove-lp}, although at the cost of longer execution times. 

==> numerical_experiments.tex <==
\section{Numerical Experiments}\label{sec:num_exp}

%Since the FPTAS algorithm is interpretable and easy to implement for practicitioners here we demonstrate how it works on real-life and synthetic examples and compare their performance with other benchmarks

\begin{algorithm}[h]
\caption{Greedy algorithm for constant move parameter version 1}\label{alg:greedy}
\begin{algorithmic}[1]
\Require graph $G$ with terminals $s_1,\ldots, s_k$ and move parameter $r$.
   \State $P_1,\ldots,P_k$ be the initial partitioning in graph $G$.% $C_0=\{(u,v)\in E(G) | \ell_u\neq \ell_v\}\gets$ initial cut-set in graph $G$. 
    \If{$r=0$}
        \State \Return the initial cut, without moving any nodes.
    \Else 
    \For{$v\in V(G)\setminus \{s_1,\ldots,s_k\}$, $j\in \{1,\ldots,k\}$}:
    \State $\delta(v,j)=\sum_{u\in P_{\ell_v}} c_{uv} -\sum_{u\in P_j}c_{uv}$.  \Comment{The amount cut value changes if node $v$ is moved from partition $\ell_v$ to partition $j$.}
    \EndFor
    \For{$i\in \{1,\ldots,r\}$}
        \State Let $(v^*,j^*)=\arg\min_{v,j}\delta(v,j)$.
        \Comment{Starting the contraction process of $v^*$ into $s_{j^*}$.}
        \For{$u\in V(G)$}:
        \State $c_{us_{j^*}}\gets c_{us_{j^*}}+c_{uv^*}$  \Comment{Updating weight of $s_{j^*}$ due to contraction.}
        \EndFor 
        \For{$v\in P_{\ell_{v^*}} \setminus \{s_{\ell_{v^*}}\}$, $j\in \{1,\ldots,k\}\setminus \{\ell_{v^*},j^*\}$}:
            \State $\delta(v,j)\gets \delta(v,j)-c_{vv^*}$. 
        \EndFor
        \For{$v\in P_{j^*} \setminus \{s_{j^*}\}$, $j\in \{1,\ldots,k\}\setminus \{\ell_{v^*},j^*\}$}:
            \State $\delta(v,j)\gets \delta(v,j)+c_{vv^*}$. 
        \EndFor
        \For{$v\in P_{\ell_{v^*}} \setminus \{s_{\ell_{v^*}}\}$}:
            \State $\delta(v,j^*)\gets \delta(v,j^*)-2c_{vv^*}$. 
        \EndFor
        \For{$v\in P_{j^*} \setminus \{s_{j^*}\}$}:
            \State $\delta(v,\ell_{v^*})\gets \delta(v,\ell_{v^*})+2c_{vv^*}$. 
        \EndFor
        \State Remove $v^*$, so $V(G)\gets V(G)\setminus \{v^*\}$.
        %\State Find non-terminal node $v$ and partition $j\in \{1,\ldots,k\}\setminus\{l_v\}$ such that moving $v$ to $j$ results in the largest reduction of cut value among all nodes and partitions.  
        %\State Contract $v$ with $s_j$ and increasing the weight of each edge $(s_j,u)$ by $c_{vu}$.
    \EndFor
    \State \Return the cut in the graph.
    \EndIf
\end{algorithmic}
\end{algorithm}

% \begin{algorithm}[h]
% \caption{Greedy algorithm for constant move parameter version 2}\label{alg:greedy}
% \begin{algorithmic}[1]
% \Require graph $G$ with terminals $s_1,\ldots, s_k$ and move parameter $r$.
%    \State $P_1,\ldots,P_k$ be the initial partitioning in graph $G$.% $C_0=\{(u,v)\in E(G) | \ell_u\neq \ell_v\}\gets$ initial cut-set in graph $G$. 
%     \If{$r=0$}
%         \State \Return the initial cut, without moving any nodes.
%     \Else 
%     \For{$v\in V(G)\setminus \{s_1,\ldots,s_k\}$, $j\in \{1,\ldots,k\}$}:
%     \State $\delta(v,j)=-\sum_{u\in P_j} c_{uv}$.  \Comment{The amount cut value may chaneg if node $v$ is moved from partition $\ell_v$ to partition $j$.}
%     \EndFor
%     \For{$i\in \{1,\ldots,r\}$}
%         \State Let $(v^*,j^*)=\arg\min_{v,j}\delta(v,j)$.
%         \Comment{Starting the contraction process of $v^*$ into $s_{j^*}$.}
%         \For{$u\in V(G)$}:
%         \State $c_{us_{j^*}}\gets c_{us_{j^*}}+c_{uv^*}$  \Comment{Updating weight of $s_{j^*}$ due to contraction.}
%         \EndFor 
%         % \For{$v\in P_{\ell_{v^*}} \setminus \{s_{\ell_{v^*}}\}$, $j\in \{1,\ldots,k\}\setminus \{\ell_{v^*},j^*\}$}:
%         %     \State $\delta(v,j)\gets \delta(v,j)-c_{vv^*}$. 
%         % \EndFor
%         % \For{$v\in P_{j^*} \setminus \{s_{j^*}\}$, $j\in \{1,\ldots,k\}\setminus \{\ell_{v^*},j^*\}$}:
%         %     \State $\delta(v,j)\gets \delta(v,j)+c_{vv^*}$. 
%         % \EndFor
%         \For{$v\in P_{\ell_{v^*}} \setminus \{s_{\ell_{v^*}}\}$}:
%             \State $\delta(v,j^*)\gets \delta(v,j^*)-c_{vv^*}$. 
%         \EndFor
%         \For{$v\in P_{j^*} \setminus \{s_{j^*}\}$}:
%             \State $\delta(v,\ell_{v^*})\gets \delta(v,\ell_{v^*})+c_{vv^*}$. 
%         \EndFor
%         \State Remove $v^*$, so $V(G)\gets V(G)\setminus \{v^*\}$.
%         %\State Find non-terminal node $v$ and partition $j\in \{1,\ldots,k\}\setminus\{l_v\}$ such that moving $v$ to $j$ results in the largest reduction of cut value among all nodes and partitions.  
%         %\State Contract $v$ with $s_j$ and increasing the weight of each edge $(s_j,u)$ by $c_{vu}$.
%     \EndFor
%     \State \Return the cut in the graph.
%     \EndIf
% \end{algorithmic}
% \end{algorithm}

\begin{algorithm}[h]
\caption{Greedy algorithm for constant move parameter version 2}\label{alg:greedy}
\begin{algorithmic}[1]
\Require graph $G$ with terminals $s_1,\ldots, s_k$ and move parameter $r$.
   \State $P_1,\ldots,P_k$ be the initial partitioning in graph $G$.% $C_0=\{(u,v)\in E(G) | \ell_u\neq \ell_v\}\gets$ initial cut-set in graph $G$. 
    \If{$r=0$}
        \State \Return the initial cut, without moving any nodes.
    \Else 
    \For{$v\in V(G)\setminus \{s_1,\ldots,s_k\}$}:
    \State $\delta(v)=-\sum_{u\notin P_{\ell_v}} c_{uv}$.  \Comment{The largest amount cut value may change if node $v$ is moved from partition $\ell_v$ to partition $j$.}
    \EndFor
    \For{$i\in \{1,\ldots,r\}$}
        \State Let $v^*=\arg\min_{v}\delta(v)$. 
        \Comment{Finding the node that has the largest contribution to cut value.}
        \For{$j\in \{1,\ldots,k\}$, $j\neq\ell_{v^*}$}.
            \State  $\delta(v^*,j)=-\sum_{u\in P_j} c_{uv}$.
        \EndFor
        \State Let $j^*=\arg\min_{j}\delta(v^*,j)$. \Comment{Finding the partition that that $v^*$ is most connected to.}
        \For{$u\in V(G)$}: \Comment{Starting the contraction process of $v^*$ into $s_{j^*}$.}
        \State $c_{us_{j^*}}\gets c_{us_{j^*}}+c_{uv^*}$.  \Comment{Updating weight of $s_{j^*}$ due to contraction.}
        \EndFor 
        % \For{$v\in P_{\ell_{v^*}} \setminus \{s_{\ell_{v^*}}\}$, $j\in \{1,\ldots,k\}\setminus \{\ell_{v^*},j^*\}$}:
        %     \State $\delta(v,j)\gets \delta(v,j)-c_{vv^*}$. 
        % \EndFor
        % \For{$v\in P_{j^*} \setminus \{s_{j^*}\}$, $j\in \{1,\ldots,k\}\setminus \{\ell_{v^*},j^*\}$}:
        %     \State $\delta(v,j)\gets \delta(v,j)+c_{vv^*}$. 
        % \EndFor
        \For{$v\in P_{\ell_{v^*}} \setminus \{s_{\ell_{v^*}}\}$}:
            \State $\delta(v)\gets \delta(v)-c_{vv^*}$. 
        \EndFor
        \For{$v\in P_{j^*} \setminus \{s_{j^*}\}$}:
            \State $\delta(v)\gets \delta(v)+c_{vv^*}$. 
        \EndFor
        \State Remove $v^*$, so $V(G)\gets V(G)\setminus \{v^*\}$.
        %\State Find non-terminal node $v$ and partition $j\in \{1,\ldots,k\}\setminus\{l_v\}$ such that moving $v$ to $j$ results in the largest reduction of cut value among all nodes and partitions.  
        %\State Contract $v$ with $s_j$ and increasing the weight of each edge $(s_j,u)$ by $c_{vu}$.
    \EndFor
    \State \Return the cut in the graph.
    \EndIf
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[h]
\caption{Greedy algorithm for constant move parameter version 3}\label{alg:greedy3}
\begin{algorithmic}[1]
\Require graph $G$ with terminals $s_1,\ldots, s_k$ and move parameter $r$.
   \State $P_1,\ldots,P_k$ be the initial partitioning in graph $G$.% $C_0=\{(u,v)\in E(G) | \ell_u\neq \ell_v\}\gets$ initial cut-set in graph $G$. 
    \If{$r=0$}
        \State \Return the initial cut, without moving any nodes.
    \Else 
    \For{$v\in V(G)\setminus \{s_1,\ldots,s_k\}$}:
    \State $\delta(v)=-\sum_{u\notin P_{\ell_v}} c_{uv}$.  \Comment{The largest amount cut value may change if node $v$ is moved from partition $\ell_v$ to partition $j$.}
    \EndFor
    \For{$i\in \{1,\ldots,r\}$}
        \State Let $v^*=\arg\min_{v}\delta(v)$. \Comment{Finding the node that has the largest contribution to cut value.}
        \For{$j\in \{1,\ldots,k\}$, $j\neq\ell_{v^*}$}.
            \State  $\delta(v^*,j)=-\sum_{u\in P_j} c_{uv}$.
        \EndFor
        \State Let $j^*=\arg\min_{j}\delta(v^*,j)$. \Comment{Finding the partition that that $v^*$ is most connected to.}
        \If{$\sum_{u\in P_{\ell_{v^*}}} c_{uv^*} +\delta(v^*,j^*)>0$}
            \State break (halt the algorithm)
        \EndIf
        \For{$u\in V(G)$}: \Comment{Starting the contraction process of $v^*$ into $s_{j^*}$.}
        \State $c_{us_{j^*}}\gets c_{us_{j^*}}+c_{uv^*}$.  \Comment{Updating weight of $s_{j^*}$ due to contraction.}
        \EndFor 
        % \For{$v\in P_{\ell_{v^*}} \setminus \{s_{\ell_{v^*}}\}$, $j\in \{1,\ldots,k\}\setminus \{\ell_{v^*},j^*\}$}:
        %     \State $\delta(v,j)\gets \delta(v,j)-c_{vv^*}$. 
        % \EndFor
        % \For{$v\in P_{j^*} \setminus \{s_{j^*}\}$, $j\in \{1,\ldots,k\}\setminus \{\ell_{v^*},j^*\}$}:
        %     \State $\delta(v,j)\gets \delta(v,j)+c_{vv^*}$. 
        % \EndFor
        \For{$v\in P_{\ell_{v^*}} \setminus \{s_{\ell_{v^*}}\}$}:
            \State $\delta(v)\gets \delta(v)-c_{vv^*}$. 
        \EndFor
        \For{$v\in P_{j^*} \setminus \{s_{j^*}\}$}:
            \State $\delta(v)\gets \delta(v)+c_{vv^*}$. 
        \EndFor
        \State Remove $v^*$, so $V(G)\gets V(G)\setminus \{v^*\}$.
        %\State Find non-terminal node $v$ and partition $j\in \{1,\ldots,k\}\setminus\{l_v\}$ such that moving $v$ to $j$ results in the largest reduction of cut value among all nodes and partitions.  
        %\State Contract $v$ with $s_j$ and increasing the weight of each edge $(s_j,u)$ by $c_{vu}$.
    \EndFor
    \State \Return the cut in the graph.
    \EndIf
\end{algorithmic}
\end{algorithm}

==> old_thm_proofs.tex <==
\subsection{$O(r^2)$-approximation algorithm for Max-$r$-move $k$-partitioning\mina{changing the algorithm}}

%\arash{ We should refer to $log(n)$-approximation algorithm for two partitions, and argue that in most cases this bound is better. If M is order O(n),  say $n/100$, then we should somehow say that greedy algorithm achieve worse that O(n) approximation. I remember Mina said the greedy has no bound. So we should say the obvious bound is worse that $M^2$ approximation. }
Let $G$ be an instance of \maxmove problem, and let $X$ be a solution to the LP relaxation of it. Let $G'$ be a subgraph of $G$ with the same vertices as $G$, and $uv\in E(G')$ if $d_X(u,v)<g$ for a given parameter $g$. We prove the following two lemmas
\begin{lemma}\label{lem:connected-comp}
If $g\le\frac{1}{8r}$ then for any two vertices $u,v$ such that $\ell_u\neq \ell_v$ and $X_v^{\ell_v},X_u^{\ell_u}\ge3/4$ we must have that $u$ and $v$ are in different connected components of $G'$. 
\end{lemma}
\begin{proof}
Let $A$ be the set of nodes $w\in G$ such that $X_w^{\ell_w}\ge 3/4$. So $u,v\in A$. By Lemma \ref{lem:size} we have that $|G\setminus A|<4r$. Suppose $u$ and $v$ are in the same connected component. There is a path $P$ in $G'$ between $u$ and $v$ in $G'$. WLOG we can assume that $u$ and $v$ are the only nodes in $P$ that are in $A$. This is because if there is $w\in A\cap P$, then either $\ell_w\neq \ell_u$ or $\ell_w\neq \ell_v$ and we consider $uw$ sub-path or $vw$ sub-path of $P$, and continue this until there is no node of $A$ in the path except for the endpoints.

Now by definition of $G'$, for every two consecutive vertices $z,z'$ on the path $P$ we have $d_{LP}(z,z')< g$. Since $d_{X}$ is the standard $L_1$ norm, it obeys the triangle inequality. So we have $d_{X}(u,v)< 4rg<1/2$ since $|G\setminus A|<4r$. Now observe that $X_v^{\ell_u},X_u^{\ell_v}\le 1/4$ and hence $d_{X}(u,v)\ge 1/2$, which is a contradiction. %So for all $u,v\in H$ we must have $\ell_u=\ell_v$. Let $i^*$ be $\ell_u$ for all $u\in H$. 
\end{proof}

Let $A$ be the set of nodes in $G$ with $X_v^{\ell_v}\ge 3/4$. By Lemma \ref{lem:connected-comp}, for every connected component $H$ of $G'$, there is an index $i_H$ such that for all nodes $v\in H\cap A$ we have $\ell_v=i_H$. Let $C_i$ be the set of connected components $H$ where $|H|>6r$ and $i_H=i$. Let $V(C_i)=\cup_{H\in C_i}V(H)$. So intuitively most vertices in $v\in V(C_i)$ we have $\ell_v=i$. Next lemma says that the number of vertices $V(C_i)$ that don't have $\ell_v$ equal to $i$ is very low. Formally if $V_i$ is all the nodes $v$ in $G$ such that $\ell_v=i$, we prove in the next lemma that $|V(C_i)\setminus V_i|$ is small. 

\begin{lemma}\label{lem:M2approx-cases}
Suppose $g\le\frac{1}{10r(r+1)(k+1)}$. For every $i=\{1,\ldots,k\}$ let $r_i=\sum_{v\in V(C_i)} (1-X_v^{\ell_v})$. Then if $C_i\neq \emptyset$, we have $|V(C_i) \setminus V_i|\le r_i+\frac{1}{k+1}$. %\mina{in the middle of changing something. }
\end{lemma}
\begin{proof}
Suppose that for some $i$, $C_i\neq \emptyset $ and
 $|C_i\setminus B_i|> r_i+\frac{1}{k+1}$. 
%Let $A$ be the set of nodes $v$ such that $X_v^{\ell_v}\ge 3/4$. By Lemma \ref{lem:connected-comp} we can't have two nodes $u,v\in A$ such that $\ell_u\neq \ell_v$. 
%So for all $u,v\in A\cap H$ we must have $\ell_u=\ell_v$. Let $i^*$ be $\ell_u$ for all $u\in A\cap H$. 
%Let $A_{i^*}$ be all the nodes $u$ with $\ell_u=i^*$. 
Observe that for each $H\in C_i$, we have $|H|>6r$. Moreover, $A\cap H \subseteq V_i$ and thus $A\cap H=V_i\cap H$. Since by Lemma \ref{lem:size} $|H\setminus A|\le |G\setminus A|<4r$, we have that $|V_i\cap H |=|A\cap H |=|H|-|H\setminus A|\ge 2r\ge 2r_i$ and $|H\setminus V_i|\le |H\setminus A|<4r$. %Since the weight of each node in the graph is at least one, $|H\setminus A_{i^*}|<4M$.

Let $v_0=\arg \min_{v\in V_i\cap V(C_i)} X_v^{i}$ and let $\alpha=X_{v_0}^{i^*}$. Let $H$ be the connected component in $C_i$ that $v_0$ belongs to. 
Let $B_1$ be the set of closest nodes in $H\cap V_i$ to $v_0$ with size at least $r_i+\frac{1}{k+1}$. Since there are less than $4r$ nodes in $H\setminus V_i$, we have that for any $v\in B_1$, the distance between $v$ and $v_0$ is at most $4r+|B_1|\le 5r+1<6r$. This means that $|X_v^{i}-X_{v_0}^{i}|\le d_X(v_0,v)\le 5rg$ and so $X_v^{i}=X_v^{\ell_v}\le \alpha+6rg$. So we have $\sum_{v\in B_1} (1-X_v^{\ell_v})> (1-\alpha-6rg)(r_H+\frac{1}{k+1})$. 

Let $B_2$ be a subset of $V(C_i)\setminus V_i$ of size at least $r_i$. For every $v\in V(C_i)\setminus V_i$, there is a node $u\in V_i$ such that $v$ is at most $4r$ away from $v$ since $|V(C_i)\setminus V_i|<4r$. So we have $|X_v^{i}-X_u^{i}|\le d_X(u,v)\le 4rg$ and thus $X_v^{i^*}\ge X_u^{i}-4rg\ge \alpha-4rg$. Since $\ell_v\neq i$, we have $\sum_{v\in B_2} (1-X_v^{\ell_v}) \ge\sum_{v\in B_2} X_v^{i}\ge (\alpha-4rg)(r_i+\frac{1}{k+1})$. So $\sum_{v\in B_1\cup B_2} (1-X_v^{\ell_v}) \ge (\frac{1}{k+1}+r_H)(1-10rg)>r_H$, where the last inequality comes from substituting the value of $g$. This is in contradiction with the definition of $r_i$ and so we must have that $|V(C_i)\setminus V_i|\le r_H+\frac{1}{k+1}$.
\end{proof}

Next we are going to put these two lemmas together to make a simple algorithm.
%\mina{$g^*$ is the integrality gap}
\msquared*

\begin{proof}
The algorithm is depicted in Algorithm \ref{alg:M2approx}.
\begin{algorithm}[h]
\caption{$O(kr^2)$-Approximation algorithm for \maxmove}\label{alg:M2approx}
\begin{algorithmic}[1]
   \State $X\gets$ solution to the LP of Table \ref{tab:maxmove-lp}. 
    \State $A\gets$ any $v\in V(G)$ with $X_v^{\ell_v}\ge 3/4$.
    %\State $A'\gets V(G)\setminus A$
    \State Create the graph $G'$: $V(G'):=V(G)$ and $uv\in E(G')$ if $uv\in E(G)$ and $d_X(u,v)<g=\frac{1}{10r(r+1)(k+1)}$.
    \For{Every connected component $H$ of $G'$}
        \State $r_H\gets \sum_{v\in H} (1-X_v^{\ell_v})$.
        \If{$|H|\le 6r$}
            \State Compute all assignments of nodes of $H$ to $k$ partitions such at at most $r_H$ nodes move. 
            \State \Return The assignment with the least cut value.
        \Else   
            \State Take an arbitrary node $v$ in $A$, let $i\gets \ell_v$.
            \State \Return The assignment where all nodes in $G$ are assigned to $i$.
        \EndIf
    \EndFor
\end{algorithmic}
\end{algorithm}
First consider a solution $X$ of the \maxmove linear program. Let $A$ be the set of nodes $v$ such that $X_v^{\ell_v}\ge 3/4$. Let $A'$ be the rest of the nodes. By Lemma \ref{lem:size}, we have that $|A'|< 4M$. %Otherwise $\sum_{u\in H'} X_u^{\ell_u}< 3|H'|/4\le |H'|-M$, and so $\sum_{v\in V(G)} X_v^{\ell_v}\le n-M$. 
We are going to make a new graph $G'$ with vertices of $G$. Let $g=\frac{1}{10M(M+1)(k+1)}$. For every $u$ and $v$, attach $u$ and $v$ in $G'$ if they are attached in $G$ and $d_{X}(u,v):=\frac{1}{2}\sum_i |X_u^i-X_v^i|< g$. %Moreover, if $u,v\in H$, then attach $u$ to $v$.  
Let $\bar{Z}$ be the optimal integer solution to the \maxmove instance. 

%\mina{If $|H'|\le M$, just put them wherever you want.}

We process each connected component individually and the final output of the algorithm is the union of the output of each connected component.

First we process the ``small" connected components of $G'$.
If $|H|\le 6M$, then by considering every combination of at most $M_H$ nodes moving, we can find the combination with least cut value. Thus if $Z$ is the solution that the algorithm finds, we have that $ \sum_{uv\in E, u,v\in H}c_{uv}d_{Z}(u,v)\le \sum_{uv\in E, u,v\in H}c_{uv}d_{\bar{Z}}(u,v)$.

For any ``large" connected component $H$ of $G'$ the algorithm takes an arbitrary node $v$ that is in $H\cap A$ and move all the nodes to $\ell_v$. We show that this actually doesn't move many nodes, and provides good approximation guarantees.

Recall that by Lemma \ref{lem:connected-comp}, for any connected component $H$ there is $i_H$ such that for all nodes $v\in H\cap A$, $\ell_v=i_H$. Let $C_i$ be the set of large connected components $H$ such that $i_H=i$. Let $M_i=\sum_{v\in V(C_i)} (1-X_v^{\ell_v})$. If $V_i$ is the set of nodes $v$ in $G$ with $\ell_v=i$, then by Lemma \ref{lem:M2approx-cases}, we have $|V(C_i)\setminus V_i|\le M_i+\frac{1}{k+1}$. So among the nodes in $V(C_i)$, at most $M_i+\frac{1}{k+1}$ nodes have been moved.

So overall only at most $M+\frac{k}{k+1}$ nodes have been moved. Note that $M$ is an integer and $M+\frac{k}{k+1}<M+1$, so at most $M$ nodes have been moved. Note that the only terminal node in $V(C_i)$ is $s_i$, and so we do not move any terminal nodes.

To evaluate the value of the cut for each large connected component $H$, note that the cut is actually zero since all nodes are in cluster $i$.

%let $Z$ denote the solution for $H$ where all non-terminal nodes go to $i$. So for any non-terminal $v$ we have $Z_v=e_{i}$. The only edges in the cut are of the form $s_jv$ for $j\neq i$, and since $X_{s_j}=e_j$, we have $d_{X}(s_j,v)\ge |X_v^{i}-X_{s_j}^{i}|=X_v^{i}\ge 3/4-M_H g$. The last inequality comes from the fact that $v$ is at most $M_H$ away from a node in $A$ due to the connectivity of $H$. By substituting $g$, we have that $d_{X}(s_j,v)\ge 1/2$. So $d_Z(s_j,v)\le 2d_{X}(s_j,v)$ and thus $\sum_{uv\in E, v,u\in H} d_Z(u,v)c_{uv}\le 2\sum_{uv\in E, v,u\in H} d_X(u,v)c_{uv}$. %Also note that we just moved at most $M$ nodes.



%$A$ is the set of closest nodes in $H$ to $v_0$, for any 
%Since $G'$ is connected, there is a node $v_1\in H$ that is attached to a node $u_1\in H'$. 
%Consider the $M$ closest nodes in $H^{i^*}$ to $v_1$, say $v_2,\ldots,v_{M+1}$. Consider $M+1$ closest nodes in $H'\setminux H^{i^*}$ to $u_1$, say $u_2,\ldots,u_{M+1}$. Let $\alpha:=X_{v_1}^{i^*}$. For each $j$, we have that $u_j$ is at most $j$ nodes away from $v_1$ in $G'$, so $X_{v_1}^{i^*}$ 


%So $|X_{v_1}^{i^*}-X_{u}^{i^*}|\le d_{LP}(v_1,u)\le g$. Since $X_{u}^{i^*}<3/4$ and $X_{v_1}$, we have $X_{v_1}^{i^*}<3/4-g$. Now consider the $8M-1$ closest nodes to $v_1$, say $v_2,\ldots,v_{8M}$. Since they are all connected, WLOG we can assume that the distance of $v_j$ to $v_1$ is at most $j-1$ and so $X_{v_j}^{i^*}<3/4-gj$. If $v_j\in H'$, then 

%So $\sum_{j=1}^{L} X_{v_j}^{i^*}< 3L/4 - g(L)(L+1)/2<L-M+1/8$. 



%We show that this graph has at least $k$ connected components. Let $H_i$ be the set of nodes $v$ in $H$ with $\ell_v=i$. Let $G_i'$ be all the nodes that have a path in $G'$ to a node in a node in $H_i$. So $H_i\subseteq G_i'$ since the nodes in $H_i$ form a clique in $G'$. We first show that $G_i'\cap G_j'=\emptyset$ for every $i\neq j$.

%Suppose that there is a node in $G_i'\cap G_j'$. So there are $u\in H_i$ and $v\in H_j$, such that there is a path $P$ between $u$ and $v$ in $G'$. WLOG we can assume that there is no vertex on this path that is in $H$ except for $u$ and $v$. So for every two consecutive vertices $z,z'$ on the path $P$ we have that one of them is not in $H$ and hence since they are connected in $G'$ we must have $d_{LP}(z,z')\le g$. Since $d_{LP}$ is the standard $L_1$ norm, it obeys the triangle inequality. So we have $d_{LP}(u,v)\le (4M-1)g<1/2$ since $|H'|\le 4M-1$. Now observe that $X_v^{\ell_v},X_u^{\ell_u}\ge 3/4$ and $\ell_u\neq \ell_v$. So $X_v^{\ell_u},X_u^{\ell_v}\le 1/4$ and hence $d_{LP}(uv)\ge 1/2$.

%\mina{the case with only one connected component: won't happen if we do 32M instead of 8M. Also then won't need recursion cause we can say the components are of size O(M). }

%Now we are ready to describe the algorithm. First we form $G'$ in $O(mk)$ time where $m$ is the number of edges of $G$. If there is only one connected component, we must have that there is $i^*$ such that for each $u\in H$, $\ell_u=i^*$, take all nodes to $i^*$. Otherwise, for each connected component $C$ of $G'$, %We redefine $G_k'$ to be all the nodes that have a path to a node in $H_k$ and any node that doesn't have any path to any of the $H_i$s. So now $G_1'\cup\ldots\cup G_k'$ contains all vertices of $G$. 
%recurse on the subgraph in $G$ induced by $V(C)$, with for a max-$\sum_{v\in C} X_v^{\ell_v}$-move $k$-partitioning. Note that the initial partitioning is part of the input of the problem, and the initial partitioning of the recursion step is the same as $G$. 

 %The base of the recursion is when the size of the graph is $O(k)$ and we can solve the problem by in $O(k^k)$ time. \mina{talk about the running time: worse case spend $O(n)$ each round, at most n rounds. and the cost of solving the LP?}

Next we prove that this algorithm has a $\frac{1}{g}+1$-approximation factor. Let $Z$ be our integer solution. Recall that $\bar{Z}$ is the optimal integer solution to the \maxmove instance. To show the approximation factor, first note that for each connected component $H$ we have 
$$
\sum_{uv\in E, u,v\in H}c_{uv}d_{Z}(u,v)\le  \sum_{uv\in E, u,v\in H}c_{uv}d_{\bar{Z}}(u,v).
$$ 
Next for each $u$ and $v$ in different connected components of $G'$ we have $d_{X}(u,v)\ge g$. So $d_{Z}(u,v)\le \frac{1}{g}d_{X}(u,v)$. Let $C(G')$ be the set of all connected components of $G'$, and let $E'$ denote the edges with endpoints in different connected components. Hence we have that 
\begin{align*}
\sum_{uv\in E}c_{uv}d_Z(u,v)&= \sum_{uv\in E'}c_{uv}d_Z(u,v)+\sum_{H\in C(G')}\sum_{uv\in E, u,v\in H} c_{uv}d_Z(u,v)\\
&\le \frac{1}{g}\sum_{uv\in E'}c_{uv}d_X(u,v)+\sum_{uv\in E, u,v\in H}c_{uv}d_{\bar{Z}}(u,v)\\
&\le (\frac{1}{g}+1)\sum_{uv\in E}c_{uv}d_{\bar{Z}}(u,v). 
\end{align*}


%Note that in each connected component $H$ we move at most $M_H=\sum_{i\in}$ nodes. Since $M\ge\sum_H M_H$, we have moved at most $M$ nodes. 

To analyze the running time, computing $G'$ using the LP solution $X$ takes linear time. If connected component $H$ is small, i.e. $|H|<6M$, then processing it takes is a function of $M$. If $H$ is large, then we only take linear time. 
\end{proof}




\subsection{$O(M)$-approximation algorithm \mina{need to change some parts of the proof.}}
%\mina{we can reduce the problem to the following: suppose the initial partitioning has all nodes in cluster 1 (except for terminal). what is the best clustering so that at most M nodes leave cluster 1?}

\begin{theorem}
Let $M$ be any positive real number. There is a $8M$- approximation algorithm for max-$M$-move $k$-partitioning in $k^{O(M^2)}T(n)$ time, where $T(n)$ is the running time of solving a linear program with $O(n)$ variables and $O(n)$ constraints. 
\end{theorem}

\begin{algorithm}[h]
\caption{Base cases}\label{alg:basecases}
\begin{algorithmic}[1]
    \State Let $A$ be all the nodes $v$ with $X_v^{\ell_v}\ge 3/4$ and $A'=V(G)\setminus A$.
    \If{$M<2$}
        \State compute the cut achieved by moving a node $v$ to any of the clusters $1,\ldots,k$.
        \State \Return The smallest cut computed.
    \ElsIf{$n<6M$}
        \State compute all cuts achieved by moving at most $M$ nodes. 
         \State \Return The smallest cut computed.
    \Else 
    \State \Return Not a base case.
    \EndIf
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[h]
\caption{$8M$-approximation algorithm for max-$M$-move $k$-cut \mina{indent cases}}\label{alg:8M_algorithm}
\begin{algorithmic}[1]
    \Require{Input graph $G$, parameter $M$}
    \State run Base Case Algorithm \ref{alg:basecases}.
    \State $X\gets$ solution to the LP of Table \ref{tab:maxmove-lp}. 
    \If{$G,M$ is a base case}
        \State \Return the output of Algorithm \ref{alg:basecases}.
    \EndIf
    \State $A\gets$ any $v\in V(G)$ with $X_v^{\ell_v}\ge 3/4$.
    \State $A'\gets V(G)\setminus A$
    \State Create the graph $G'$: $V(G'):=V(G)$ and $uv\in E(G')$ if $uv\in E(G)$ and $d_X(u,v)<g=\frac{1}{8M}$.
    

    \State We have the following cases:
    \State \textbf{Case 1.} $G'$ has more than one connected component
    \For{each connected component $H$ of $G'$}
            \State Recurse on $H$ with move parameter $\sum_{v\in H}(1-X_v^{\ell_v})$, let $Z_H$ be the recursion solution.
            \State \Return $Z = \cup_H Z_H$.
        \EndFor
    
    \State Let $i^*$ be the cluster where for all $v\in A$, $\ell_v=i^*$ \Comment{such cluster exists when $G'$ has one connected component}
    \State \textbf{Case 2.} $G'$ has one connected component and for all $v\in A'$, $\ell_v=i^*$. 
            \State \Return the solution $Z$ where $Z_v=e_{i^*}$ for all non-terminal nodes $v$.
    \State \textbf{Case 3.} $G'$ has one connected component and $|A'|\le M$
    %\State Let $i^*$ be the cluster such that for all non-terminal $v\in A$, $\ell_v=i^*$.
        \State \Return $Z$ where for all $v\in G$, $Z_v=e_{i^*}$.
    \State \textbf{Case 4.} $G'$ has one connected component and $|A'|\ge \floor{M}+1$
        \For{All assignments $Y_v$ of vertices of $A'$ to the $k$ partitions $\{e_1,\ldots,e_k\}$ such that $\sum_{v\in A'}Y_v^{\ell_v}\ge |A'|-M$}
            \For{All $i\in \{1,\ldots,k\}$}
            \State $A_i'\gets $ all nodes $v\in A'$ that are assigned to cluster $i$, i.e. $Y_v=e_i$.
            \EndFor
        \State $M'\gets \sum_{v\in A'}(1-Y_v^{\ell_v})$ is the number of nodes in $A'$ that are moved.
        \State Create the graph $H^{(Y)}$ by contracting each set $A_i'\cup \{s_i\}$ into a new node $s_i^*$
        \State Let $Z^{(Y)}$ be the solution to the recursion on $H^{(Y)}$ with the move parameter $M-M'$. Extend $Z^{(Y)}$ from $H^{(Y)}$ to $G$ below.
        \For{All $i\in \{1,\ldots,k\}$}
            \For{All $v\in A_i\cup s_i$}
            \State define $Z^{(Y)}_v=e_i$
            \EndFor
        \EndFor
        \EndFor
    \State \Return $Z^{(Y)}$ that minimizes the cut over all $Y$.
    
\end{algorithmic}
\end{algorithm}






\begin{proof}
We first describe our algorithm along with intuitions for different steps, and then prove the approximation guarantees of it. The base cases of our algorithm is depicted in Algorithm \ref{alg:basecases} and the main algorithm is in Algorithm \ref{alg:8M_algorithm}.

First we consider that $M\ge 2$. Otherwise for each non-terminal node $v$ and each cluster $i$, compute the cut obtained by moving $v$ to cluster $i$. Among all these cuts and the initial cut, output the one that is smallest. This is the first case in Algorithm \ref{alg:basecases}.

So from here we assume that $M\ge 2$.
Consider a solution $X$ of the max-$M$-move $k$-partitioning linear program. Let $A$ be the set of nodes $v$ such that $X_v^{\ell_v}\ge 3/4$. Let $A'$ be the rest of the nodes. By Lemma \ref{lem:size}, we have that $|A'|< 4M$.

We create a graph $G'$ with the same vertices as $G$ as follows. Let $g=\frac{1}{8M}$ be a gap parameter. For every $u$ and $v$, attach $u$ and $v$ in $G'$ if they are attached in $G$ and $d_{X}(u,v):=\frac{1}{2}\sum_i |X_u^i-X_v^i|< g$. From here we have three cases.
\begin{itemize}
    \item \textbf{Case 1.} Suppose $G'$ has more than one connected component. Then we recurse on each component $H$ with move parameter $M_H:=\sum_{v\in H}(1-X_v^{\ell_v})$. The base case of this recursion is when $H<6M$. The output solution is  the union of the solutions of each component.
    
    If $G'$ is connected, by Lemma \ref{lem:connected-comp}, for every $u,v\in A$, if $\ell_u\neq \ell_v$ then $u$ and $v$ are in different connected components in $G'$. So there is a $i^*$ such that for all $v\in A$, $\ell_v=i^*$.
    \item \textbf{Case 2.} Suppose that $G'$ is connected and for all $v\in A'$, $\ell_v=i^*$. In this case we don't move any nodes, so the solution $Z$ that the algorithm outputs is $Z_v=e_{i^*}$ for all non-terminal nodes $v$.
    \item \textbf{Case 3.} Suppose that $G'$ is connected and $|G'\setminus A|=|A'|\le M$. In this case we move all non-terminal nodes to $i^*$.
    \item \textbf{Case 4.} Suppose that $G'$ is connected and $|A'|\ge \floor{M}+1$. Consider all assignments of nodes in $A'$ to the $k$ clusters such that at most $M$ of them move from their primary cluster. There are at most $k^{|A'|}<k^{4M}$ such assignments. For each assignment, we are going to decide how to move the remainder of the nodes which are the nodes in $A$ recursively as follows. Consider an assignment $Y$ of nodes in $A'$, and suppose that $M'\le M$ nodes have been moved. 
    For each $i$ let $A_i'$ be the nodes in $A'$ that are assigned to cluster $i$. ``Contract" all these nodes with $s_i$, the terminal in cluster $i$, and call this ``super-node" $s_i^*$. For each node $u\notin A_i'$ define the $s_i^*u$ weight $c_{s_i^*u}=\sum_{v\in A_i'\cup \{s_i\}}c_{vu}$. Let the resulting graph be $H^{(Y)}$ with terminals $s_1^*,\ldots, s_k^*$ and with move parameter $M-M'$. 
Since $|A'|>1$, the number of nodes in $H$ is less than $G$, and we can recurse on $H$. 

The base of the recursion consists of three cases. The first two cases are when $M<2$ and when $n<6M$ which are described above. The third case is when all nodes $v\in A'$ also have $\ell_v=i^*$. For this special case of input, we don't recurse on the configuration where none of the nodes in $v$ move. Formally, consider the configuration $Y$ where for all nodes $v\in A'$ we have $Y_v=e_{\ell_v}$. We won't recurse on $H^{(Y)}$. Instead, we output the solution where we move no nodes. All the other base cases are depicted in Algorithm \ref{alg:basecases}.

We then output the solution with the least cut among all the configurations as the final solution of our algorithm. Note that for any configuration that we recurse on, if $Z$ is the solution this instance, then for any $u$ that is contracted into $s_i^*$ we let $Z_u=Z_{s_i^*}$.
\end{itemize}
The approximation factor is proved to be $8M$ in Lemma \ref{lem:approx-guarantee}
 and the running time of the algorithm is proved in Lemma \ref{lem:runningtime}.
%Now the running time of this case is at most $k^{4M}F(n-1)$. The running time of the algorithm is dominated by this step, and so we have $F(n)\le T(n)+k^{4M}F(n-1)$ \mina{not complete}
\end{proof}

\begin{lemma}\label{lem:approx-guarantee}
Algorithm \ref{alg:8M_algorithm} is a $8M$-approximation algorithm for max-$M$-move $k$-partitioning.
\end{lemma}
\begin{proof}\mina{change the Y in prelim.}
Let $Z$ be the solution of our algorithm and let $\bar{Z}$ be the optimal integer solution. Let $X$ be the optimal LP relaxation solution of the \maxmove instance. \mina{fix this} If $G'$ is not connected (Case 1), then for each connected component $H$ we have $\sum_{vu\in E(H)} c_{uv}d_Z(u,v)\le \frac{1}{g}\sum_{vu\in E(H)} c_{uv}d_{\bar{Z}}(u,v)$. This is because if $X'$ is an LP solution for $H$, then $\sum_{vu\in E(H)} c_{uv}d_X(u,v)\ge \sum_{vu\in E(H)} c_{uv}d_{X'}(u,v)$, and from recursion assumption we have that $\sum_{vu\in E(H)} c_{uv}d_Z(u,v)\le \frac{1}{g}\sum_{vu\in E(H)} c_{uv}d_{X'}(u,v)$. Now for each $u$ and $v$ that are not in the same connected component we have that $d_X(u,v)>g$, so $d_Z(u,v)\le \frac{1}{g}d_X(u,v)$. So the cut value created by $Z$ is at most $\frac{1}{g}=8M$ times the value of the cut created by the LP solution. Note that the max move condition is equivalent to $\sum_v (1-X_v^{\ell_v})\le M$, so we have $\sum_H M_H\le M$ and we have moved at most $M$ nodes.

So suppose that $G'$ is connected. In this case by Lemma \ref{lem:connected-comp} there is a node $i^*$ such that for all non-terminal nodes $v\in A$, $\ell_v=i^*$ \mina{make sure you always say non-terminal}. First suppose that for all $v\in A'$, $\ell_v=i^*$ (Case 2). In this case the solution of the algorithm is $Z_v=e_{i^*}$ for all non-terminal nodes $v$. Any cut in this solution is of the form $us_i$ where $i\neq i^*$. Now since $|A'|<4M$, any node $u$ is either in $A$ or is at most $4M$ edges away from $A$ in $G'$. If $v$ is the closest node in $A$ to $u$, then we have $d_X(u,v)\le 4gM<1/2$, so $|X_u^{i^*}-X_v^{i^*}|\le 1/2$. Thus we have $X_u^{i^*}\ge 1/4$. So $d_X(u,s_i)\ge |X_u^{i^*}-X_{s_i}^{i^*}|\ge 1/4$, and we have $d_Z(u,s_i)\le 4d_X(u,s_i)$. So the cut that $Z$ creates has value at most four times the cut that the LP creates.

Now suppose that $|A'|\le M$ (Case 3). In this case the algorithm moves all the nodes in $A'$ to $i^*$, and so any edge in the cut is of the form $us_i$ for $i\neq i^*$. For any non-terminal $u$, either $u$ is in $A$ or is connected to a node in $A$ with a path of length at most $M$. So $X_u^{i^*}\ge 3/4-Mg>1/2$. 
Since $X_{s_i}=e_i$, $d_X(u,s_i)\ge 1/2$ and so $d_Z(u,s_i)\le 2d_X(u,s_i)$. So the cut value created by $Z$ is at most twice the cut value that $X$ represents. So $Z$ is in fact a $2$-approximation. 

Finally suppose that $|A'|\ge \floor{M}+1$ (Case 4).
Let $\bar{Z}$ be the optimal integer solution to the problem. We have considered the case where we partition the nodes in $A'$ exactly like $\bar{Z}$. Let the graph resulting from the contractions be $H$. Note that if we contract nodes $u$ a $v$ into $s_i^*$ for some $i$, it must be that $\bar{Z}_v=\bar{Z}_u=i$. 
Recall that $A_i'$ is the set of all the nodes contracted into $s_i^*$. By defining $Y_{s_i^*}=e_i$ we see that the value of the cut that $Y$ represents in $G$ doesn't change in $H$, i.e. $\sum_{uv\in E(G)}c_{uv}d_{\bar{Z}}(u,v) = \sum_{uv\in E(H)}c_{uv}d_{\bar{Z}}(u,v)$. Let $\bar{Z}_H$ be the optimal integer solution for $H$. So we have $\sum_{uv\in E(H)}c_{uv}d_{\bar{Z}}(u,v)\ge \sum_{uv\in E(H)}c_{uv}d_{\bar{Z}_H}(u,v)$. Moreover, from recursion, if $Z$ is the solution that the algorithm outputs, we have $\frac{1}{g}\sum_{uv\in E(H)}c_{uv}d_{\bar{Z}_H}(u,v)\ge \sum_{uv\in E(H)}c_{uv}d_{Z}(u,v)$. So we have 
\begin{align*}
\frac{1}{g}\sum_{uv\in E(G)}c_{uv}d_{\bar{Z}}(u,v) = 
    \frac{1}{g}\sum_{uv\in E(H)}c_{uv}d_{\bar{Z}}(u,v)\ge \sum_{uv\in E(H)}c_{uv}d_{Z}(u,v) = \sum_{uv\in E(G)}c_{uv}d_{Z}(u,v)
\end{align*}
Note that for the last equality we used the fact that for all the nodes $u$ contracted into $s_i^*$, we let $Z_u=Z_{s_i^*}$. So $Z$ is a $\frac{1}{g}$-approximation. 
\end{proof}
\begin{lemma}\label{lem:runningtime}
Algorithm \ref{alg:8M_algorithm} runs in time $k^{O(M^2)}T(n)$ where $T(n)$ is the running time of solving a linear program with $O(n)$ variables and $O(n)$ constraints. 
\end{lemma}
\begin{proof}
Let $F(n,M)$ be the running time of Algorithm \ref{alg:8M_algorithm} on instances of \maxmove on instances with $n$ nodes. We show that $F(n,M)\le k^{O(M^2)}O(T(n))$, where $T(n)$ is the running time of solving a linear program with $O(n)$ variables and $O(n)$ constraints. We assume that if $n_1+n_2=n$, $T(n_1)+T(n_2)\le T(n)$, and that $T(n)\ge n$. 

In fact we prove that $F(n,M)\le 2k^{4M(M-1)}T(n)$.
First consider the special instances where there is $i^*$ such that for all non terminal nodes $v$ we have $\ell_v=i^*$. Let the running time of this case be denoted by $F'(n,M)$. First note that any instances produced in the algorithm to recurse on is of this type. To see this, observe that the recursions only happen on case 1 and case 4. In case 1, each connected component of $G'$ will also have all non-terminal nodes initially belonging to $i^*$. and in case 4, in any assignments of nodes in $A'$ to clusters, all the nodes that haven't been contracted are a subset of non-terminal nodes in $G$ so they all  non-terminal nodes in those graphs also initially belong to $i^*$.

We show that $F'(n,M)\le T(n)k^{2M(M-1)}-2$, and to do that we recurse on $M$.

For case 1 of the algorithm we have that $F'(n,M)\le \sum_H F'(|H|,M_H)$ where the sum is on the connected components $H$ of $G'$, and we have $\sum_H |H|=n$ and $\sum_H M_H\le M$. Since $T(n)\ge \sum_H T(n_H)$ and $m_H\le M$ for all $H$, we have $F'(n,M)\le T(n)k^{2M(M-1)}-2$. 

Case 2 and 3 have linear running times. So suppose that we are in case 4 of the algorithm. Recall that we consider all assignments of nodes in $A'$ to clusters $1,\ldots,k$ such that at most $M$ of them move from their original clusters. For the assignment where every node in $A'$ is assigned to its initial cluster, the recursion stops in case 2, since all nodes are from cluster $i^*$. 

For all the other assignments, at least one node in $A'$ is assigned to a cluster other than its initial cluster. Moreover the size of these graphs are at most $n-1$, since $A'>1$.
So we have $F'(n,M)\le k^{4M}+k^{4M}F'(n-1,M-1)$. The first term is due to the comparison of results at the end. We also assume that $O(n)\le k^{4M}F'(n-1,M-1)$, since the algorithm takes linear time to read the input. By our recursion on $M$, we have that $F'(n-1,M-1)\le k^{2(M-1)(M-2)}T(n-1)-2$. So we have $F'(n,M)\le k^{4M}+k^{2M(M-1)}T(n-1)-2k^{2M(M-1)}\le k^{2M(M-1)}T(n)-2$.% (we used the fact that $2k^{2M(M-1)}-k^{4M}\ge 2$.

%(say we use the fact that $F(n,M)\ge F(n',M')$ for $n\ge n'$ and $M\ge M'$).
Now to prove the bound on $F$, we use a similar approach. We use a recursion on $M$. Cases 1,2 and 3 are the same as above. To analyze case 4, first consider the assignment that assigns all nodes in $A'$ to their initial partition. The graph resulting from contracting nodes in this case has all non-terminal nodes belonging to a cluster $i^*$, and so the running time is at most $F'(n-1,M)$. For all the other assignments, we have at least one node in $A'$ that is assigned to a partition other than its initial partition, and so the max move parameter of the resulting graph is at most $M-1$.

So we have that $F(n,M)\le F'(n-1,M)+ k^{4M}F(n-1,M-1)\le k^{2M(M-1)}T(n)+k^{4M}F(n-1,M-1)$. Using recursion assumption on $M$, we have that $F(n-1,M-1)\le 2k^{4(M-1)(M-2)}T(n-1)\le 2k^{4(M-1)(M-2)}T(n)$, and so $F(n,M)\le T(n)(2k^{4(M-1)(M-2)}+k^{2M(M-1)})\le 2k^{4M(M-1)}T(n)$. 
\end{proof}


==> oldintro.tex <==



%\mina{STOC doesn't have any formats or limits. IPCO does though, 12 pages max in their specific format.}
%\mina{some relevant info that would help in writing the story is in related work subsection} 


\section{Introduction}
%\section{Problem Definition and Motivation}
\mina{motivations added somewhere, use cases etc.}

\mina{graph $k$-partitioning doesn't have terminals, we should avoid using it.}
%\mina{generally graph partitioning is used in VLSI layout, parallel computing, machine learning (for what tasks), etc}
%Given a graph $G$ and an integer $k\ge 2$ the \textit{graph $k$-partitioning} problem asks to find a partitioning of the nodes of $G$ into $k$ partitions, such that the sum of the weight of the edges that are between two different partitions, aka \textit{the cut value}, is minimized. The \textit{multiway cut} problem is graph $k$-partitioning with terminal. Given $k$ terminals, the problem asks to find a partitioning of nodes into $k$ partitions such that each partition has exactly one terminal, and the cut value is minimized among all $k$-partitionings with exactly one terminal in each partition. It is known that for $k>2$, multiway cut is APX-hard \cite{nphardmultiwaycut}.
Graph partitioning problem is one of the most fundamental and widely used graph problems in computer science. A \textit{$k$-partitioning} of a graph $G$ refers to partitioning its nodes into $k$-disjoint sets, or \textit{partitions}, and often the goal is to find a $k$-partitioning with the least \textit{cut value}\footnote{also referred to as \textit{cut size}} which is the sum of the edges that are between different partitions.
Graph partitioning is used in machine learning, parallel computing, computer vision, VLSI design and many more areas \cite{vision,parallel1,learning,vlsi}.

Given a graph $G$, an integer $k\ge 2$ and $k$-terminals, the famous \textit{multiway cut} problem asks to find a partitioning of the nodes of $G$ into $k$ partitions, such that the sum of the weight of the edges that are between two different partitions, aka \textit{the cut value}, is minimized, among all $k$-partitionings that have exactly one terminal in each partition. It is known that for $k>2$, multiway cut is APX-hard \cite{nphardmultiwaycut}. 

we define and study a natural variant of the multiway cut problem called \textit{\maxmove}. Suppose that we are given a graph $G$ with an initial $k$-partitioning, an integer $k\ge2$, $k$ terminals and a \textit{max move parameter} $r\in \mathbb{Z}$. The problem only considers $k$-partitionings such that at most $r$ non-terminal nodes have been moved from their initial partition. The \maxmove problem asks to find a $k$-partitioning that minimizes the cut value over all the $k$-partitionings considered. Similarly we define \textit{exact-$r$-move $k$-partitioning} problem, where we consider the $k$-partitionings with exactly one terminal in each partition such that ``exactly" $r$ nodes have moved from their initial partition.


Numerous examples of the \maxmove problem can be seen in real world networks. In fact, in a lot of networks, the underlying graph already has a $k$-partitioning, and the goal is to improve the cut value of this $k$-partitioning by moving ``a few" nodes around. For example consider a company with many branches across the country. One way to make the distribution of employees more efficient is to have the employees that communicate a lot with each other in the same office. This also decreases the fragmentation of different groups across offices, as the employees in a team tend to have high amount of communication with each other than with members of other teams. So if we model the company structure using a graph where the nodes are the employees and the edge weights are proportional to the amount of communication between them, we seek a $k$-partitioning with a low cut value, where $k$ is the number of offices. 

However, no company has the budget to do a big reorganization, and can only move a certain number of employees. Moreover, not all employees can move. We can model these employees with the terminal nodes, by ``contracting" all the employees in an office (partition) that cannot move into a terminal node for that office. So if the company budget dictates that at most $r$ employees can be relocated, then we seek a \maxmove where the initial partitioning is the distribution of people in the offices. 

As another example, consider \mina{homeless people problem}

%We define and study a natural variant of the multiway cut problem

There has been a long line of work providing approximation algorithms for multiway cut \cite{nphardmultiwaycut,LP_paper,angelidakis2017improved,vazirani,ugchardness} \mina{add more?}, most of which use a simple linear programming (LP) relaxation of the problem called the \textit{CKR LP }\footnote{also referred to as the earthmover LP in \cite{ugchardness}}, in honor of the authors—Calinescu, Karloff and Rabani—who introduced it \cite{LP_paper}. The best approximation factor for multiway cut is $1.2965$ due to Sharma and Vondrak \cite{bestapprox} who round the CKR LP. Interestingly Manokaran et al \cite{ugchardness} showed that assuming unique games conjecture \cite{ugc}, if the integrality gap of the CKR LP is $\alpha$, multiway cut cannot be approximated better than $\alpha$. Berczi et al \cite{berczi2020improving} showed that the integrality gap of the CKR LP is at least $1.20016$, and hence showing that the best approximation factor for multiway cut lies between $1.20016$ and $1.2965$. Closing this gap is one of the oldest open problems. 
% \mina{what is integrality gap lower bound then? 1.20016}

\mina{add sentences like it is still open for .. problem whether .. }
%\mina{motivations here in this paragraph} In a lot of applications, we have an initial $k$-partitioning, and we want to ``optimize" the cut of this $k$-partitioning without moving too many nodes around.


Perhaps the closest known variant of the multiway cut problem to \maxmove problem is the \textit{min $s$-$t$ cut with at most $r$ vertices} also known as \textit{\stcutatmost} problem\cite{zhang2016new}. This problem asks to find an $s$-$t$ cut where there are at most $r$ nodes in the $s$-side, where the $s$-side refers to the partition containing $s$. This problem is a special case of max-$(r-1)$-move $2$-partitioning when in the initial partitioning all non-terminal nodes are in the $t$-side. By moving at most $r-1$ nodes to the $s$-side, the $s$-side will have size at most $r$.
One interesting observation is that \stcutatmost doesn't have any natural extensions to $k$-partitions, however our problem is not dependent on the value of $k$.

Even though \stcutatmost is a variant of $st$-cut which is polynomially solvable, \stcutatmost is NP-complete \cite{chen2016size}, and thus \maxmove[2] and \maxmove are NP-complete. It is also known that this problem admits a \textit{Fixed Parameter Tractable (FPT)}\footnote{A problem of size $n$ and parameter $r$ is said to be FPT if there is an algorithm that solves it in $f(r)O(n^c)$ time, where $f$ is any function and $c$ is a constant independent of $r$.} solution with parameter $r$ when the graph is unweighted \cite{lokshtanov2013clustering}\footnote{The \stcutatmost problem is called \textit{cutting at most $r$ vertices by edge-cut with terminal}}. Intuitively one might wonder if \maxmove[2] and \stcutatmost are in fact equivalent. We show that \maxmove[2] is in fact W[1] hard and thus we resort to approximation algorithms for \maxmove for all $k\ge 2$. The main theme of our paper is around the following question.

\begin{center}
    \textit{How well can we approximate \maxmove?}
\end{center}

\mina{like we want to take the initial step in solving this problem}
%We show that interestingly we can match the best approximation factor for \stcutatmost to \maxmove[2]. Moreover for $k>2$, we show 
%Moreover, there is no problem that is this similar to \maxmove for $k>2$, and so 
%which we are given a graph $G$ with initial $k$ partitions and an integer $M$ \mina{maybe r?}, and we want to achieve the smallest cut by only moving $M$ nodes from their initial clusters. Note that here the cut for $k$ partitions means the sum of pairwise cuts between every pair of partitions. When we require at most $k$ \elaheh{shouldn't be $M$?} moves from the initial partitioning, we call the problem \textit{max-$M$-move $k$-partitioning} or \textit{max-$M$-move $k$-way cut} and when we require exactly $k$ \elaheh{shouldn't be $M$?}\mina{yeah there are some places that i mix up k and M, haven't changed them cause i dont like M either} nodes to be moved we call the problem \textit{exact-$M$-move $k$-partitioning} or \textit{exact-$M$-move $k$-way cut}.

%\mina{check the correct name of max m s-t min cut}
%When $k=2$, there are many similar problems to $M$-move $2$-partitioning that has been studied. In max-$M$ $st$-min cut, we are looking for cut with $s$-side having at most $M$ nodes \mina{cite}. This problem is a special case of max-$M$-move $2$-partitioning when initially all nodes except $s$ are in the $t$-cluster. This problem is also known as \textit{cutting at most $M$ vertices by edge-cut with terminal} and is known to be NP-complete and fixed parameter tractable when parameterized by $M$ \elaheh{notation they use is $M$?}\mina{They use k cause they are in the 2-partitioning case} or the size of the cut \mina{cite}. From the similarity of these problems the following questions come up.


\subsection{Our results}
\mina{say:our results may not be tight but none of the similar partitioning variants have tight results showing that this problem is hard. even the multiway cut itself is not tight.}
First we consider the $k=2$ case. We show that weighted \stcutatmost, unweighted \maxmove[2] and subsequently \maxmove for $k>2$ are all W[1]-hard with by a polynomial reduction from densest $r$-subgraph. It is well-known that densest $r$-subgraph with parameter $r$ is W[1] hard \cite{densest}.

\begin{restatable}{theorem}{w1hardness}\label{thm:w1hard}
Min $r$-size $s$-$t$ cut and \maxmove with parameter $r$ are W[1]
 hard.
\end{restatable}

Next we extend the CKR linear program to an LP for \maxmove by adding a linear constraint that reflect the move constraint we have in the problem. Using this LP, we show that we can get similar approximation guarantees as the result of \cite{zhang2016new}, which is a $\frac{r+1}{r+1-r^*}$-approximation algorithm for \stcutatmost in $O(nm\log^n/m)$ time, where $r^*$ is the size of the $s$-partition of the optimal cut. To prove this result, \cite{zhang2016new} also extends the CKR linear program to an LP for \stcutatmost. They use the result of \cite{gallo1989fast} on parametric flows which dominates and indicates their running time of $O(mn\log^2(n)/m)$\footnote{It is possible that with the progress on max flow algorithms this algorithm could run faster}. However our result is independent of \cite{gallo1989fast}(See section \ref{sec:tech-overview}).

\begin{restatable}{theorem}{thmtwopart}\label{thm:2part}
There is an approximation algorithm that solves weighted $n$-node $m$-edge instances of \maxmove[2]with approximation factor $\frac{r+1}{r+1-r^*}$, where $r^*$ is the size of the optimal solution. 
It runs in time $O(n)T_{mincut}(m)$ where $T_{mincut}(m)$ is the running time of the $st$ min-cut algorithm on a $m$-edge graph.
\end{restatable}

Note that due to Chen et al \cite{chen2022maximum} the best running time for max flow/min cut problem is $m^{1+o(1)}$ time so our algorithm is in time $O(n\cdot m^{1+o(1)})$.

We show that the \maxmove LP that we use to prove Theorem \ref{thm:2part} has integrality gap at least $r+1$ for all $k\ge 2$. \cite{zhang2016new} shows that the \stcutatmost LP has integrality gap at least $\frac{r}{2}$. We show that the weighted version of \stcutatmost has integrality gap $r+1$ as well. Since $\frac{r+1}{r+1-r^*}\le r+1$, this means that the integrality gap for \stcutatmost is exactly $r+1$, since the algorithm of \cite{zhang2016new} works for weighted graphs.

Next we present our main result, which is an approximation algorithm for \maxmove for $k>2$. We essentially round the \maxmove linear program in linear time and give a $O(kr^2)$-approximation algorithm for it.

\begin{restatable}{theorem}{msquared}\label{thm:m2approx}
Let $OPT$ be the value of the optimal cut of \maxmove returned by its LP relaxation, for a given positive integer $r$. There is an algorithm for \maxmove on $m$-edge graphs with approximation factor $10kr(r+2)$ in $T(n)+O(mk)$ time where $T(n)$ is the running time of solving a linear program with $O(n)$ variables and $O(n)$ constraints. 
\end{restatable}

\begin{corollary}
Let $g^*$ be the integrality gap of the \maxmove LP. Then $r+1\le g^*\le 10kr(r+2)$.
\end{corollary}

Since the integrality gap is at least $r+1$, we cannot hope for an approximation algorithm with constant factor. However, we show that if the optimal cut value that \maxmove LP outputs is OPT, if we violate the max move constraint by a constant factor, i.e. allow to move $c\cdot r$ nodes for some constant $c$, then we can find a $k$-partitioning with cut value at most a constant factor of OPT. 

\begin{restatable}{theorem}{fourmove}\label{thm:fourM}
Let $OPT$ be the value of the optimal cut of \maxmove returned by its LP relaxation. 
Then there is an algorithm that rounds the \maxmove LP and obtains an integral solution with value at most $3OPT$ by moving at most $4r$ nodes. %\arash{better this way? or removing the LP to make it more appealing ? }
\end{restatable}

Finally we discuss the shortcomings of linear programming to capture all problem properties, and show that a quadratic program formulation of the problem has integer optimal solution, and could be used to solve the problem exactly\footnote{Not necessarily in polynomial time, however softwares such as CPLEX are very fast in solving quadratic programs.}.








% \subsection{2-partitioning}
% We show that unweighted max-$\nu$-move $2$-partitioning is W[1] hard. We also show that min st cut with at most $\nu$ vertices is W[1] hard when the graph is weighted. Note that this problem is FPT when unweighted.

% Moreover we show that the cardinality gap for both problems is $\nu+1$ (weighted case).

% We extend the $\frac{\nu+1}{\nu+1-\nu*}$-approx algorithm of \cite{zhang2016new} to max-$\nu$-move $2$-partitioning. 

% \subsection{$k>2$}
% \mina{gonno put theorems here}
% %This problem can be defined as a special case of semi-supervised graph partitioning which we describe in the next subsection, and there are no theoretical results for it.
% %Also in theory cs there are many problems that are special cases of this problem such as min-$k$ $s-t$ cut that is a special case of max-$k$-move $2$-partitioning.  


% Our hardness result also shows that min st cut with at most k vertices on ``weighted graph" is W[1] hard! 

% Our integrality gap example also works for min s-t cut with at most k vertices. The previous result showed k/2 integrality gap and we show k+1 integrality gap which matches their approx algorithm.
\subsection{related work \mina{shorten?}}
First we should mention that the version of the multiway cut without the terminals is the $k$-partitioning problem which asks to divide the nodes of a graph into $k$ partitions such that the resulting cut value is minimized. Similar to the multiway cut problem, the $k$-partitioning problem is polynoimally solvable for $k=2$ and NP complete for $k>2$.

There are many variants of the multiway cut and $k$-partitioning problems in the literature, we name a few that are variants with additional size constraints. As mentioned before the \stcutatmost problem is NP-complete even though the min-cut problem with one side having at most $k$ nodes is polynomially solvable\cite{armon2006multicriteria,watanabe1987edge}. Note that \stcutatmost is the terminal version of this problem. 

The exact version of the \stcutatmost problem is called \textit{Min E$r$-Size $s$-$t$ cut}\cite{feige2003cutting} which asks to find an $s$-$t$ cut with minimum cut value among all the cuts that have exactly $r$ nodes in the $s$-side. The \textit{$(r,n-r)$-cut} \cite{bonnet2015multi} is the above problem without terminals $s$ and $t$ and asks for a cut with minimum value over all cuts with one side having exactly $r$ nodes. $(r,n-r)$-cut is known to be W[1] hard\cite{bonnet2015multi}, and as a result Min E$r$-Size $s$-$t$ cut is W[1] hard. For both problems there is a randomized $O(r/\log(n))$ algorithm due to \cite{feige2003cutting}. These problems have been studied when parameterized by cut value as well \cite{fomin2013parameterized}.
 
The \textit{$(k,\nu)$-balanced graph partitioning} problem asks to partition the graph into $k$ partitions such that the cut is minimized over all the $k$-partitionings with each partition having at most $\nu\cdot \frac{n}{k}$ nodes.  \cite{andreev2004balanced} gives a bi-criteria polynomial time approximation algorithm with $O(\log^2n)$ approximation factor for constant $\nu>1$. For $\nu=1$ there is no approximation algorithm with finite approximation factor unless $P=NP$ even for $k=2$ (see \cite{garey1979guide}). \mina{any balanced versions of multiway cut??}

\mina{talk about submodular multiway cut?}

%$k$-partitiong and multiway cut problems are used extensively in machine learning. 
 
%\textbf{2 partitions}: 
%\begin{itemize}
    %\item Size constraint on the s-side of the s-t cut: minimum s-t cut with at least k vertices, minimum s-t cut with at most k vertices, minimum st cut with exactly k vertices: all NP-complete \cite{chen2016size}. for the ``at most k" version, there is a $\frac{k+1}{k+1-k^*}$ approx $O(mn\log{n^2/m})$ time algorithm where $k^*$ is the optimal cut \cite{zhang2016new}. 
   % \item min cut with one side having at most $k$ nodes is polynomialy solvable (\cite{armon2006multicriteria,watanabe1987edge}) but when you add terminals (s,t), it becomes NP-complete as mentioned above.
   % \item ``Cutting at most $k$ vertices by edge-cut with terminal" \cite{fomin2013parameterized,lokshtanov2013clustering} is exactly "the min s-t cut with at most $k$ vertices". \cite{lokshtanov2013clustering} show that it is FPT when parameterized by k, when the graph is unweighted! 
    %\item We show that min $s-t$ cut with at most $M$ vertices is a special case of 2 partitioning with max move. To see this, the initial cluster for all nodes except $s$ is called Cluster $2$ and the initial cluster of $s$ is Cluster $1$. $s$ and $t$ are our two terminals. $2$-partitioning with move parameter $M$ is min $s-t$ cut with at most $M$ vertices. our results related to the stuff here: we show that even though min $s-t$ cut with at most $M$ vertices is FTP, our problem is W[1] hard. However, it still gets a $\frac{M+1}{M+1-M^*}$-approximation \elaheh{$M^*$ is the optimal number of vertex moves?}\mina{yeah the optimal solution moves at most $M$ nodes, suppose it moves exactly $M^*$ nodes}.
    
    %\item ``min cut with exactly k vertices" or min $(k,n-k)$-cut is W[1] hard (\cite{bonnet2015multi} gives this citation for it \cite{downey2003cutting,cai2008parameterized}\mina{I did a quick check and couldn't pin down the result in either of the papers.}). This is a non-terminal version, it is NOT min s-t cut with exactly $k$ vertices. Though it also shows that the s-t version must be W1 hard: suppose it is FPT. So for every pair of s and t solve the terminal version and take the best cut, this just adds a $n^2$ factor. \\
    %Also for both terminal and non-terminal version there is a randomized $O(k/log n)$ algorithm due to \cite{feige2003cutting}.
    %\item might not need to include this: \cite{fomin2013parameterized} also considers the following problem: Given a graph $G$ and integers $k,t$, find a vertex set $X$ with $|X|\le k$ and $|N(X)|\le t$, where $N(X)$ is the set of neighbors of $X$. They show that the problem is FPT when parameterized by $t$ but $W[1]$ hard when parameterized by $k$. For the terminal variant, the problem is W[1] hard when parameterized either by $k$ or by $t$ alone but FPT when parameterized by $k+t$. Note that they are considering $N(X)$ to be the vertex neighborhood of $X$ not the edge neighborhood. It's interesting that the vertex neighborhood version is hard and the edge neighborhood is FPT.

%\end{itemize}
%$(k,n-k)$ cut, cutting at most k vertices by edge cut with/without terminal. 

%\textbf{k partitions}: 
% \begin{itemize}
%     \item $(k,v)$-balanced graph partitioning, where you want the min cut with each partition having at most $v\cdot \frac{n}{k}$ nodes. \cite{andreev2004balanced} gives a bi-criteria polynomial time approximation algorithm with $O(\log^2n)$ approximation factor for constant $v>1$. For $v=1$ there is no approximation algorithm with finite approximation factor unless $P=NP$. \mina{i think this is without terminals}
%     \item \mina{didn't search a lot, someone maybe do it?}
%     \item \mina{is there any problem equivalent to this: all nodes are in one cluster at first (and we have terminals) we want to move at most M nodes out of this cluster to other clusters to minimize the cut}
% \end{itemize}
%\paragraph{k-partitioning work in ML}
$k$-way partitioning and multiway cut problems are extensively used in machine learning and there are many heuristics used in practice for solving them such as the Kernighan-Lin (KL) algorithm \cite{kl-alg,fiduccia} for $k=2$, Spectral clustering \cite{ng2001spectral}, kernel $k$-means \cite{kkmeans} and many other (see \cite{survey}). %While algorithms such as kernel $k$-means extend naturally to $k>2$, for many other $2$-partitioning specific algorithms such as the KL algorithm the problem is generalized to $k>2$ by a recursive bisection \cite{survey}.
%A lot of algorithms for $k>2$ is applying a bisection algorithm recursively. \cite{survey} is a survey from 2015 on graph partitioning.

Moreover, variants of the $k$ partitioning problem such as \textit{semi-supervised $k$-way partitioning} problem have been fairly studied by which one could formulate the multi-way cut problem.   %\textit{semi-supervised $k$-way partitioning} problem. 
In the semi-supervised setting of the $k$-partitioning problem, we have limited supervision in terms of pairwise constraints, typically ``must-link" and ``cannot-link" constraints limiting pairs of nodes to be in the same partition or in different partitions \cite{kulis2009semi}.% These constraints are represented as a set of pairs of nodes. Formally, if $(u,v)$ is in the must-link set, $u$ and $v$ must be in the same partition, and if it is in the cannot-link set, $u$ and $v$ cannot be in the same partition. 

%\mina{i agree with you that having must-link constraints is unnecessary. I think people mention it to treat it as a "soft" constraint since it is an NP problem anyway.}

%This problem has been fairly studied, for example \cite{kulis2009semi} encodes the constraints in the kernel matrix of the kernel $k$-means \cite{kkmeans}.


%\cite{chen2016size} shows that $s-t$ cut with size constraints is NP-complete. The size constraints are at most $k$, at least $k$ and exact $k$, meaning that the set that $S$ is in must have size at most $k$, etc. The problem is NP-complete for any of these constraints. We call the at most $k$ and exact $k$ problems by \textbf{min-$k$ s-t cut} and \textbf{exact-$k$ s-t cut}. Of course when $k$ is bounded by a constant the problem is polynomially solvable so this is for $k$ that is not constant.



%\cite{zhang2016new} gives a $\frac{k+1}{k+1-k^*}$-approximation $O(mn\log{n^2/m})$ time algorithm for min $k$ s-t cut, where $k^*$ is the size of the optimal cut. Note that $k^*\le k$ so the approximation factor is at most $k$. 

%For exact $k$ s-t cut, there is a randomized $O(k/\log n)$ algorithm  \cite{feige2003cutting}.

%Interesting fact: min-$k$ cut (not s-t cut) is polynomially solvable. So having fixed nodes s and t make the problem NP complete.


%In exact-$M$ s-t cut, the problem looks for a cut that has exactly $M$ nodes in the s set. \cite{feige2003cutting} gives a $O(k/\log n)$ approximation algorithm: The algorithm has two stages: contraction stage and combining stage. In contraction stage we select an edge randomly (with probability proportional to its weight) and contract it. Note that initially the weight of each node is 1 and when we contract two nodes of weight $w1$ and $w2$ the weight of the new node is $w1+w2$. In combining stage, using dynamic programming we select a subset of nodes with total weight exactly $M$ with minimal degree. For example if all the nodes have weight one, we simply select the $M$ nodes with smallest degree. 

%This is a randomized algorithm a 
%nd the $\log n$ appears because of the probability of success. If $k=\Omega{\log{n}}$ the approximation is good, if $k$ is small they don't talk about the approximation factor so it is probably not great.

%\subsubsection{known hardness results}
%The problem of min $(k,n-k)$ cut is W[1] hard (\cite{bonnet2015multi} provides citations), this is the non terminal version of exact-$k$ st cut which is a special case of exact-$k$-move 2-partitioning.

%\cite{fomin2013parameterized} considers the following problem: Given a graph $G$ and integers $k,t$, find a vertex set $X$ with $|X|\le k$ and $|N(X)|\le t$, where $N(X)$ is the set of neighbors of $X$. They show that the problem is FPT when parameterized by $t$ but $W[1]$ hard when parameterized by $k$. For the terminal variant, the problem is W[1] hard when parameterized either by $k$ or by $t$ alone but FPT when parameterized by $k+t$. Note that they are considering $N(X)$ to be the vertex neighborhood of $X$ not the edge neighborhood.

%The problem of ``cutting at most k vertices by edge-cut with terminal" seems to be min k s-t cut, and \cite{lokshtanov2013clustering} proves it to be fixed-parameter tractable when parameterized by $k$ or $t$. The general problem they solve is as follows: In $(\mu, p,q)$-partition problem, the task is to find a partition of vertices into clusters where each cluster $C$ satisfies the requirements that (1) at most $q$ edges leave $C$ and (2) $\mu(C)\le p$, where $\mu$ is an arbitrary polynomial time compatible monotone function like the size of $C$. They show that there are $2^{O(p)}n^{O(1)}$ and $2^{O(q)}n^{O(1)}$ algorithms for this problem. \mina{I don't know how they go from this problem to the min k-st cut problem but apparantly they do, have to read it. it is probably via the below idea}

% \subsubsection{useful idea}
% \begin{definition}
% Let $S\subseteq E$ be an $st$ cut, and let $K$ be the component of $G\setminus S$ containing $s$. We say that $S$ is an important $s-t$ cut if it is inclusionwise minimal and there is no $st$ cut $S'$ with $|S'|\le |S|$ such that $K\subset K'$ for the component $K'$ of $G\setminus S'$ containing $s$.
% \end{definition}
% Then they show the following:
% \begin{lemma}\cite{lokshtanov2013clustering}
% For every $k$, there are at most $4^k$ important $st$ cuts of size at most $k$, and we can find them in $4^kn^{o(1)}$ time.
% \end{lemma}

%It's interesting that the vertex neighborhood version is hard and the edge neighborhood is fpt. Can we say that our problem is w1 hard as well? we prove this in the next section.



%\paragraph{Some facts about densest subgraph} (we might not use these at all.) \cite{manurangsi2020strongish} showed that there is no algorithm with running time $f(k).n^{O(1)}$ for densest $k$-subgraph with approximation factor $o(k)$ under Strongish planted clique hypothesis. A previous result under Gap-ETH exists for approx factor $k^{o(1)}$.

%Moreover, \cite{manurangsi2017almost} shows that there is no polynomial time  $n^{(\frac{1}{\log\log n})^c}$-approximation algorithm for densest-$k$-subgraph under ETH. Note that $c>0$ is a universal constant (Note that this is not parameterized)


%\arash{ Wouldn't be easier to set $Z^i_v=0$ when $v \in X'_j$ and $j \ne i$ ? }
%\majid{We only need to define $Z^i_v$ for nodes that are not colored. I fix the formulation. }

\subsection{Organization of the paper}
\mina{to be filled}

==> other.tex <==

\subsection{Most general setting}
\mina{should be simplified wrt what we eventually prove}
\begin{problem}{Minimum Cost list partition problem}
We are given a graph $G$ together with non-negative weight function $w : V(G) \times V(G) \rightarrow \mathbf{Q}_{\ge 0}$.
Each node $x \in G$ has list of possible colors/partitions, $L(x) \subset \{1,2,\dots,k\}$.  
%The goal is to find a list-partitioning of $G$ so that each node is assigned to one of the 
%partition from its list, and the total weight of the edge across different partitions is minimized. 
The goal is to find a mapping $\rho : V(G) \rightarrow \{1,2,\dots,k\}$, so that 
for every $x \in G$, $\rho(x) \in L(x)$ and $\sum\limits_{x,y \in G , \rho(x) \ne \rho(y)} w(x,y)  $ is minimized. 
\end{problem}

\paragraph{ Special setting and application:}
Our setting differs from the usual partitioning problems by the initial partitioning. We are given an initial partitioning together with the network. Some of the nodes in the network cannot be moved from their clusters. The rest of the nodes can be moved to any other cluster. We can easily formulate these constraints with must-link and cannot-link constraints (or equivalently lists). The initial objective is to minimize the pairwise cut of the partitions. 

Note that for each initial cluster, one can aggregate all the nodes that cannot be moved from this cluster into one super-node, so we are only left with cannot-link constraints among the pairs of super-nodes.

\paragraph{Additional constraints for the practical setting} The following constraints are not necessary to begin with but would be great to apply. Each cluster has a cost, and so we want to avoid moving nodes from low cost to high cost clusters unnecessarily, so we need to add a penalty for this in any objective function. 

Additionally, we want the algorithm to be able to get the number of nodes we would like to move as input, and move only that many nodes while minimizing the objective. 

\arash{Additionally, we want the algorithm to be able to put a limit on the  relocation cost. In other words, for each move from cluster $i$ to cluster of $j$ there is a cost (in a simple case the cost would be $1$). More precisely, we are given a cost function $\mu : [1,k] \times [1,k] \rightarrow  \mathbf{Q}_{\ge 0} $ where $\mu(i,i)=0$. }

Therefore, the goal is to find a mapping $\rho : V(G) \rightarrow \{1,2,\dots,k\}$, so that 
for every $x \in G$, $\rho(x) \in L(x)$ and $\sum\limits_{x,y \in G , \rho(x) \ne \rho(y)} w(x,y) $ is minimized. Moreover, 
$\sum\limits_{x,y \in G} \mu(\rho(x), p(y)) \le M$. 


\subsection{Rounding of \cite{LP_paper} with list restrictions - ideas}

The list conditions are translated in to $X_u^i=0$ for pairs of $u$ and $i$. In the rounding process, we can still subdivide nodes and the solution to the new graph works for the old graph, since we don't change $X_u$ for any original node $u$. 

Note that the only time that the rounding scheme can violate a list restriction is when $\rho$ is big that all entries of a node $u$, and so $u$ can end up in cluster $k$, and it might be that $X_u^k=0$ and hence violating the list restrictions. There are the following fixes to this:
\begin{enumerate}
    \item Let $k$ be the cluster that everyone can go to, i.e. we don't have $X_u^k=0$ restriction for any $u$. Note that using this solution we only get a $1.5$ approx and not a $1.5-1/k$. This fix is especially possible if we have a cheap country that everyone can go. 
    \item \mina{todo, need to do more analysis on rounding}
\end{enumerate}
\subsection{Our problem: Limiting number of moves}
We add the following constraint to the last LP. Let $\ell_v$ be the initial location of $v$. Let M be the maximum number of moves allowed.
\begin{equation}\label{eq:maxmove}
    \sum_{v\in V-S} X_{v}^{\ell_v} \ge |V-S|-M
\end{equation}
 
Recall that we call this problem \textbf{Max-$M$-move $k$-partitioning}. If we have equality in the above, then the problem is called \textbf{exact-$M$-move $k$-partitioning}.

In rounding of the LP with the max move condition, when going from $\rho=1$ to $\rho=0$, the number of moves decreases \textbf{if we fix the ordering of clusters}. Recall that in rounding we either start to fill cluster $1$ and go up to $k-1$, or we start to fill cluster $k-1$ and go down to $1$.

When $\rho=1$, all nodes that can move go to cluster $k$. If node $u$ has moved to cluster $i\neq k$ for $\rho = \rho_1$, then if $\rho_2<\rho_1$, since the ordering is fixed, node $u$ is again going to move to cluster $i$. Now some nodes that went to cluster $k$ with $\rho_1$ might now go to another cluster with $\rho_2$.


Note that if the ordering is not fixed, node $v$ might move to some location $i\neq l_v$ with $\rho_1$, where $l_v$ is the initial location of $v$. But then with $\rho_2$ and a different ordering, it might move to $l_v$, and hence it is possible that the number of nodes moved decreases when allowing the ordering to change.

Questions:
\begin{enumerate}
    %\item In the rounding (of the LP with max move constraint), in the experiments on MS data as we grow $\rho$ the number of people moved grows. Can we prove that this happens?
    \item If there is $m<M$ such that there is a solution with $m$ moves that reduces the cut of the initial clusters, the is there a $\rho$ that gives a solution with $m'<M$ moves? ANSWER: No, the bad example doesn't do this. 
    \item same question as above for $m=M$ and $m'=M$. ANSWER: NO, bad example.
\end{enumerate}

\subsection{bad example}

%\arash{As far as I can see the optimal solution is to move $w$ to cluster $2$ and get the cut value $21$. While the fractional LP value could be setting $X_u^1=X_u^2=X_v^1=X_v^2=0.5$. In this case the cut value would be $10(1-X_u^1)+10(1-X_v^1)+5+1(1-0.5)+1(1-0.5)=16$. Therefore, the integrality gap is $21/16=1.3125 <1.5$ but more than $1.30$ (the approximation bound in Vondrak's paper) but still less than $1.5$. }

%\mina{please see "integrality gap" section to see why the gap can be very large. }
%\arash{ I calculate the integrality gap this way: (The optimal solution of the problem) / ( the optimal fractional LP). Thus, we should try to find some fractional values for the LP to make the objective function value as small as possible (minimization in our case). In Figure 1, the integrality gap is not big according to those fractional values.  If we remove vertex $w$ from the graph then the optimal does not move any vertex at all (because we put a bound on the number of moves and we don't want to achieve the exact number of moves). So, the optimal is $20$ and the fractional values for LP could be $X_u^1=X_u^2=X_v^1=X_v^2=0.5$, and the fractional LP value is $11$, and hence, the integrality gap is $20/11 < 2$. Perhaps, this is a good example because it shows the integrality gap could be bigger than $1.5$. Maybe you mean different values for the LP. Do you think there is another example or should we put a collection of these examples to get a bad example? } \mina{for exact max move condition the integrality gap is huge, but for non exact as you said it is not, and i don't think there is any bad example for it.}

In Figure \ref{fig:bad_example}, the LP with max move parameter set to 1 will have the following solution: $X_u^1 = X_u^2 = X_v^1 = X_v^2 = 0.5$, and the rest of the nodes will stay wherever they are. Note that by moving $u$ and $v$ together to cluster 2, the cut value is going to be $7$, whereas by moving $w$ to cluster 2, the cut will be $21$ (hence reduced by 4). Now to round this solution we need to move either $u$ or $v$ to cluster 2, and in any case the cut is going to be more than $W$. 


\begin{figure}
    \centering
    \includegraphics{bad_example_LP.eps}
    \caption{}
    \label{fig:bad_example}
\end{figure}
Basically the problem is that the distance between $u$ and $v$ for the solution of the LP is zero, even though it should be $W/2$.

Note that in case of no max move constraints, the rounding works because if $X_u=X_v$ then they end up in the same cluster, and if $X_u\neq X_v$ then the distance between $u$ and $v$ is not zero. 


\subsection{Practical solutions implemented so far}
\begin{itemize}
    \item For $k=2$, the Kernighan-Lin algorithm gives good results and we can apply the constraints mentioned, however for $k>2$ it is very inefficient.
    \item Kernel k-means is more efficient for any $k$ though it is hard to apply the cannot-link constraints in it. The algorithm of \cite{kulis2009semi} for applying the constraints gives very weak solutions.
    \item Any spectral clustering algorithm that needs computing eigenvalues (of the Laplacian usually) is very inefficient, though any new tricks for computing eigenvalues fast is appreciated.
    % 
\end{itemize}



\section{Other LPs}
\subsection{LP formulation using network flows strategy}
Let $X_i$ be the set of nodes that their color can change and they get color $i$ after optimization (go to partition $i$) for $i\in\{1\cdots k\}$.
Let $X_i'$ be the set of fixed nodes that have to stay in partition $i$.

For each non-fixed node $v$ and color $i$ define variables $Z^i_v$ as follows:
\begin{equation*}
  Z^i_v  =
    \begin{cases}
      1 & \text{if $v \in X_i$}\\
      0 & \text{otherwise}
    \end{cases}       
\end{equation*}
For each edge $uv\in E$ define variables $d_{uv}$ as follows:
\begin{equation*}
  d_{uv}  =
    \begin{cases}
      0 & \text{if $u,v \in X_i \cup X'_i $ for some $i\in\{1\cdots n\}$}\\
      1 & \text{otherwise ($uv$ is in the cut)}
    \end{cases}       
\end{equation*}

  
\begin{table}[hht]
    \centering
    \begin{tabular}{lllr}
    \toprule
        \texttt{Minimize:} & $\sum_{uv\in E}c_{uv}d_{uv}$ & &\\
        \texttt{Subject to:} & & &\\
        & $d_{uv}\ge Z^i_u - Z^i_v$  & for all  $uv\in E$ for all $i\in\{1\cdots n\}$,  & (C1)\\
        & $d_{sv}\ge 1 - Z^i_v$ & for all $sv\in E$ for all $i\in\{1\cdots n\}$ for all $s\in X'_i$ & (C2)\\
        & $d_{ut}\ge Z^i_u$ & for all $ut\in E$ for all $i\in\{1\cdots n\}$ for all $t\in \cup_{j \neq i}X'_j$ & (C3)\\
        & $d_{st}\ge 1$ & for all $st\in E$ for all $s\in X'_i,t\in X'_j$ for all $ i,j\in\{1\cdots n\},i\neq j$ & (C4)\\
        & $\sum_{i=1}^k Z^i_v = 1$ & for all $v$ & (C5)\\
        \bottomrule
    \end{tabular}
    \caption{LP 1}
    \label{tab:Majids-lp}
\end{table}


\subsection{LP formulation using Sherali-Adam's type constraints }
For every pair of vertices $x,y \in G$ and every $i,j \in \{1,2\dots,k\}$ we define variable $xy_{ij}$ when $i \in L(x)$ and $j \in L(y)$. If $xy_{ij}=1$ then we $x$ is mapped to partition $i$ and $y$ goes to partition $j$. If $xy_{ij}=0$ then either $x$ doesn't map to partition $i$ or $y$ doesn't map to partition $j$. Let $p(x) \in \{1,2,\dots,k\}$ denote the initial partion of $x \in G$.


\begin{table}[hht]
    \centering
    \begin{tabular}{lllr}
    \toprule
        \texttt{Minimize:} & $\sum\limits_{uv \in E \ \ i \ne j \in [1,k]} c_{uv}X_{(u,i),(v,j)}$ & &\\
        \texttt{Subject to:} & & &\\
        & $X_{(u,i),(v,j)}= X_{(v,j),(u,i)}$ & for all $u,v \in G$,  & (C1)\\
        & $X_{(u,i),(v,j)} + X_{(w,l),(v,k)} \le 1$ & for all $u,v \in G$ and $k \ne j$ & (C2)\\
        & $\sum\limits_{ \substack {i \in L(u),j \in L(v) }} X_{(u,i),(v,j)}=1$ & for all $u$ and $v$ in $G$ & (C3)\\
         & $\sum\limits X_{(u,i),(v,j)} \le \max({M \choose 2},1)$ \mina{might need changing} & 
         for all $u$ and $v$ in $G$ and every $i \ne \ell_u$ and $j \ne \ell_v$& (C4)\\

        \bottomrule
    \end{tabular}
    \caption{LP2 % \mina{C4 is wrong. it is because xy variables are for edges so the sum on the left hand side can be much bigger than M even if we move only M nodes. Example: Assume that M is 4 and we have two clusters and we move 4 nodes ($x,y,u,v)$ that are initially in cluster 1 to cluster 2. So the left hand side of C4 is at least $xy_{22}+xv_{22}+xu_{22}+yu_{22}+yv_{22}+uv_{22}=6$. I think if we replace $M$ with ${M \choose 2}$ it works.}
    %\arash{ I agree.. it should be replaced by something else, but not sure about ${M \choose 2}$ }
    }
    \label{tab:sherali-adams-lp}
\end{table}

\subsection{bad example}
Short story: we make another lp from lp2 to make it more constrained, and prove that actually this new lp admits all the fractional solutions to the paper lp, which means that we have the same problems for it. Below I describe this new lp.


The new lp comes from attempts to round lp2. We need to make up variables $Y_u^i$ for each node $u$ that corresponds to the fraction of $u$ in location $i$. Ideally $X_{(u,i),(v,j)}=Y_u^iY_v^j$, and so we also need this consistency constraint: $\sum_{j\in L(v)} X_{(u,i),(v,j)} = Y_u^i$ for all $v$. We also need that $\sum_{i\in L(u)}Y_u^i=1$ which means that (C2) is redundant, because $X_{(u,i),(v,j)}\le Y^j_v$ and $X_{(w,l),(v,k)}\le Y^k_v$ and the sum of the right hand side in these inequalities is zero because of our new conditions. Namely, we would get at this LP.

\begin{table}[hht]
    \centering
    \begin{tabular}{lllr}
    \toprule
        \texttt{Minimize:} & $\sum\limits_{uv \in E \ \ i \ne j \in [1,k]} c_{uv}X_{(u,i),(v,j)}$ & &\\
        \texttt{Subject to:} & & &\\
        & $X_{(u,i),(v,j)}= X_{(v,j),(u,i)}$ & for all $u,v \in G$,  & (C1)\\
        & $\sum_{j\in L(v)}X_{(u,i),(v,j)}=Y^j_u $ & for all $u,v \in G$& (C2')\\
        & $\sum_{i\in L(u)} Y_u^i = 1 $ & for all $u$ in $G$ & (C3')\\
         & $\sum\limits X_{(u,i),(v,j)} \le {M \choose 2}$ & 
         for all $u$ and $v$ in $G$ and every $i \ne \ell_u$ and $j \ne \ell_v$& (C4)\\

        \bottomrule
    \end{tabular}
    \caption{LP2}
    \label{tab:sherali-adams-lp-new}
\end{table}

%However, we can still have bad examples for this


\paragraph{any solution to Table \ref{tab:sherali-adams-lp-new} is a solution to Table \ref{tab:sherali-adams-lp}.} To see this, Note that (C2') and (C3') result in (C3) in Lp2. Moreover as said above, they give (C2) as well. 

To produce the bad example, We want to have one move, so we should change C4 to the left hand side $\le 1$.

The same bad example works here. Namely, the LP would set $X_{(u,1),(v,1)}=X_{(u,2),(v,2)}=1/2$ and $X_{(u,2),(v,1)}=X_{(u,1),(v,2)}=0$. The rest of the variables have are defined as follows: for each node $z$ that is not $u$ and $v$ if $z$ is in location $i$, let $Y_z^i=1$ and the other $Y$ variable be zero. Let $Y_u^1=Y_v^1=Y_u^2=Y_v^2=1/2$. Now for each edge $zt\neq uv$, define $X_{(z,i)(t,j)}=Y_z^iY_t^j$.  
This solution produces the same value for the objective as the paper LP. while the right solution is to move $w$.

%\iffalse 



\section{Quadratic Program}
We change the distance measure to $d(u,v) = 1-\sum_i X_u^iX_v^i$. So the Quadratic Program is as follows:
\begin{table}[hht]
    \centering
    \begin{tabular}{lllr}
    \toprule
        \texttt{Minimize:} & $\sum_{uv\in E}c_{uv}d_{uv}$ & &\\
        \texttt{Subject to:} & & &\\
        & $d_{uv}= 1-\sum_i X_u^iX_v^i$  & for all  $uv\in E$ for all $i\in\{1\cdots k\}$,  & (C1)\\
        & $d_{uv}= \sum_{i\neq j} X_u^iX_v^j$  & for all  $uv\in E$ for all $i\in\{1\cdots k\}$,  & (C1')\\
        & $\sum_{i=1}^{k}X^i_u=1$ & for all $u\in V$ for all $i\in\{1\cdots k\}$ & (C2)\\
        & $X_{s_i}=e_i$ & for all $s_i\in S$  & (C3)\\
        & $\sum_{v\in V-S} X_{v}^{\ell_v} \ge |V-S|-M$ & &(C4)\\
        \bottomrule
    \end{tabular}
    \caption{QP, note C1 and C1' are equivalent and either can be used.}
    \label{tab:QP1}
\end{table}


% \begin{table}[hht]
%     \centering
%     \begin{tabular}{lllr}
%     \toprule
%         \texttt{Minimize:} & $\sum_{uv\in E, i \ne j}c_{uv}u_iv_j$ & &\\
%         \texttt{Subject to:} & & &\\
%         & $u_i=\delta_{i\ell_u}$ & for all $u\in S$, $i \in [1,k]$ & (C1)\\
%         & $\sum_{i=1}^k u_i=1$ & for all $u\in V/S$ & (C2)\\
%         & $\sum_{\substack{u\in V/S\\i: i\neq \ell_u\\}} u_i \leq M $ & & (C3)\\
%         \bottomrule
%     \end{tabular}
%     \caption{\mina{equivalent to the QP above}}
%     \label{tab:QP2}
% \end{table}




The intuition behind the new distance function is that if $u$ is in $i$ with fraction $X_u^i$ and $v$ is in $j$ with fraction $X_v^j$, then the weight of $uv$ between $u$ in $i$ and $v$ in $j$ is $X_u^iX_v^j$. So the contribution of edge $uv$ is $\sum_{i\neq j}X_u^iX_v^j = 1-\sum_i X_u^iX_v^i$. Let $S$ be the set of fixed nodes.
%Note that the integrality gap in this example is not bigger than 2, and it can be achieved by increasing the weights of $uRest_2$ and $vRest_2$. 


\begin{lemma}
Let $X$ be a fractional solution to the quadratic program without C4 (the constraint with $M$, the max move parameter). Let $v$ be a node of the graph and let $i$ and $j$ be two locations, such that $X_v^i>0$ and $X_v^j>0$. Then changing $X_v^i$ and $X_v^j$ such that $X_v^i+X_v^j$ remains the same doesn't change the objective value of the QP. 
\end{lemma}

\begin{proof}
First note that changing $X_v^i$ and $X_v^j$ such that $X_v^i+X_v^j=p_1+p_2$ is fixed only affects the cut between location $i$ and $j$. The cut between $v$ in $i$ and $j$ is $\sum_{u\in j} c_{uv}X_u^jX_v^j = X_v^i \sum_{u\in j}c_{uv}X_u^j$. Let $\alpha := \sum_{u\in j}c_{uv}X_u^j$, so the cut is $X_v^i\alpha$. Similarly if we define $\beta := \sum_{u\in i}c_{uv}X_u^i$, we have that the cut between $v$ in $j$ and $i$ is $X_v^j\beta$. Note that $X_v^i\alpha$ and $X_v^j\beta$ are the only terms in the objective $\sum_{uv\in E} c_{uv}d_{uv}$ that might change. 

If $\alpha < \beta$, then by changing $X_v^i=p_1+p_2$ and $X_v^j = 0$, the cut decreases. Similarly we cannot have $\beta < \alpha$. So we have $\alpha = \beta$. Thus changing $X_v^i$ and $X_v^j$ as long as $X_v^i+X_v^j$ remains the same doesn't affect the objective
\end{proof}

\mina{basically this is why we mostly get integer solutions anyway cause $\alpha=\beta$ happens very rarely in a real world graph.}

\begin{corollary}
If $X_v$ has non-zero entries at locations $i_1,\ldots, i_t$, we can choose any of the locations $i_j$, let $X_v^{i_j}=1$ and the rest of the entries of $X_v$ be zero. Then the objective value in unchanged, all constraints are satisfied except possibly C4.
\end{corollary}


\begin{theorem}
Given a fractional solution $X$ to the QP we can round it such that the objective value does not change.
\end{theorem}

\begin{proof}
%First if there is a $v$ with a fractional $X_v$ such that $X_v^{\ell_v}=0$, just choose any of the non-zero entries of $X_v$ and make that one and make the rest zero. This satisfies C4 because $v$ is in $V-S$ and $X_v^{\ell_v}$ remains zero.
Let $S'$ be the set of nodes where $X_v^{\ell_v} = 1$. Note that $S\subseteq S'$. So C4 is equivalent to $\sum_{v\in V-S'} X_v^{\ell_v} \ge |V-S'|-M$. Note that for all $v\in V-S'$ we have that $X_v^{\ell_v}<1$. Now let $T$ be an arbitrary set of $|V-S'|-M$ many nodes $v\in V-S'$ with $X_v^{\ell_v}>0$.
Note that because $\sum_{v\in V-S'} X_v^{\ell_v} \ge |V-S'|-M$, there number of nodes $v$ with $X_v^{\ell_v}>0$ is at least $|V-S'|-M$ and we just take $|V-S'|-M$ many of them and put those nodes in $T$.

For all $v\in T$, change $X_v^{\ell_v}$ to $1$ and the rest of the entries of $X_v$ to zero. For any $v$ in $V-S'$ and outside $T$, take $i\neq \ell_v$ such that $X_v^i\neq 0$ and set $X_v^i$ to one, and the rest of the entries of $X_v$ to zero. This change satisfies C4 and doesn't change the objective. 
\end{proof}

\fengpei{The above proof might be invalid. The objective might change. The claim it does not change relies on Lemma 2.1 whose proof might no longer hold in the presence of constraint (C4). Basically, in the presence of (C4), you might not be able to move a fraction solution (without decrease the objective) to a integer one without violating (C4) or decrease the objective?, thus the addition of Lemma 2.1 on top of this might not hold? 
Check the following arguments: I believe using the arguments from Lemma 2.1, for a given $u$, we can argue the solution either satisfies 1) $u_i\in\{0,1\}$ and $\sum_{i=1}^k u_i=1$ (call the set of such nodes $S_1$) or 2) $u_{\ell_u}+u_i=1$ for some $i\neq \ell_u$ (call this index $\ell'(u)$) with $u_{\ell_u},u_i>0$ and $u_j=0$ for other $j\notin\{\ell(u),\ell'(u)\}$ (call the set of such nodes $S_2$). For $u\in S_2$, $\frac{\partial \text{obj}}{\partial u_{\ell'(u)}}$, the gradient of objective w.r.t $u_{\ell'(u)}$ must be strictly smaller than $\frac{\partial \text{obj}}{\partial u_{\ell'(u)}}$, otherwise we can make $u\in S_1$.  If $S_2$ is not empty (we show this is a contradiction), in this case, we could argue that we must have $\sum_{u\in S_2} u_{\ell'(u)}$ equals an integer, otherwise the objective can still decrease strictly ( $(C4)$ would not be tight when the sum is a fraction and the gradient difference is strict, we can decrease objective by moving the value of $u_{\ell(u)}$ towards $u_{\ell'(u)}$). Then, we can compare the value in the set $\{\frac{\partial \text{obj}}{\partial u_{\ell(u)}}-\frac{\partial \text{obj}}{\partial u_{\ell'(u)}}\}_{u\in S_2}$. If we let $u^*=\argmax_{u\in S_2}\frac{\partial \text{obj}}{\partial u_{\ell(u)}}-\frac{\partial \text{obj}}{\partial u_{\ell'(u)}}$, we can set $u^*_{\ell'(u^*)}=1,u^*_{\ell(u^*)}=0$ and $u_{\ell'(u)}=0,u_{\ell(u)}=1$ for $u\in S\{u^*\}$. This would not increase the objective and we can eliminate $S_2$. }

\fengpei{I also think we can may argue (using the same argument based on gradient) all the local optimal solution has is an integer solution? Then the fact that we kept getting optimal solution likely is that the starting state is more or less close to optimal... a.k.a the current assignment is not far from optimally efficient... But, in order to avoid possible bad optimization scenario, I recommend the following SDP relaxation(in the next section), which should always provide a valid lower bound.  }


\arash{ This is a good point that SDP avoids bad examples. }



\arash{ We should try to round LP number 2. I believe it implies LP 1,3. Can we show its integrality gap is at most $k^2$ ? Any constant approximation would be interesting.} 
%\arash{Isn't it better to use LP5. I am not sure we can solve the LP in polynomial time. It is convex?
%The rounding can't be that easy. Doesn't change C4 in LP4 (C3 in LP5)? By increasing $X^i_v$ the number of moves may increase. %}\mina{it is convex. C4 might change but there is an easy fix for that, I will write it later. If we remove C4, i claim that rounding is easy, and it gives noreduction in cut.} 
%\mina{LP 4 and LP 5 are equivalent btw. }

In terms of the running time, it seems that if quadratic program objective is $X^TQX+c^TX$, then if $Q$ is positive definite there is a polynomial algorithm (fo und a $n^4$ one for $n$ variables from long time ago, might be faster now). 

Our $Q$: $Q_{(u,i), (v,j)}$ is $c_{uv}$ if $i\neq j$ and is zero otherwise. Also assuming that $c_{uu}=0$.

\mina{Our $Q$ has real eigenvalues but since the trace of $Q$ in our problem is zero, it has negative eigenvalues as well. generally QP with $Q$ having even one negative eigenvalue is NP-hard \cite{pardalos1991quadratic}}

\majid{In Table \ref{tab:QP1} $Q_{(u,i), (v,j)}$ is -$c_{uv}$ if $i = j$ and is zero otherwise. 
For this problem to be convex the matrix $C$ should be negative semi-definite which is not the case.
We can turn this problem into a convex problem by adding self loops. 
To do so we make the matrix $C$ \textbf{diagonally dominant} by adding self loops with negative weights to the graph 
$c_{uu}=-\sum_{v\in V} c_{uv} $. 
This modification adds $-\sum_{u \in V} c_{uu}\sum_i {X_u^i}^2$ to the objective which is not desirable 
however it makes the problem convex and solvable in polynomial time.
Please note that integer solutions to Problem \ref{tab:QP1} with and without self loops are the same.
}


\mina{from CPLEX documentation, it should terminate if the QP is not semi-positive definite, unless we specify the ``optimality targer" parameter (link: ``https://www.ibm.com/docs/en/icos/12.10.0?topic=qp-distinguishing-between-convex-nonconvex-qps") Though i didn't specify such a thing and it works. I think Docplex looks for the globally optimum solution by default.}

\majid{If you define your variables as continuous variables then CPLEX gives you an error that the problem is not convex }

%\mina{If rounding doesn't change the cut and all weights are positive then we can solve partitioning in polynomial time which is not true because it is NP (is it NP for positive weighted graphs?) for fixed k the problem can be solved in poly time tho. }

Quadratic program in partitioning references that might be useful:
\begin{itemize}
    \item ``Quadratic Programming Techniques for Graph Partitioning" (didn't find a citation for it in google scholar): improves KL by using a quadratic program to switch nodes between 2 partitions.
    \item \cite{QP1} didn't read it but didn't see a k-clustering QP in the first glance.
    \item \cite{QP2} This paper has a maximization QP that I think can be converted into our QP. Upon first glance they don't talk about rounding or runtime or being convex. They talk about having size constraints for each cluster, though they say they don't consider such constraints in their QP. 
    
    \item \fengpei{Related to \cite{hager2015continuous,povh2007copositive,burer2009copositive}. In the paper \cite{burer2009copositive}, quadratic programming with binary variable and linear equality constraints (equality only) is shown to be equivalent to a linear program over the dual of the cone of
copositive matrices. This is still NP-hard but it is a convex program.}
\item \fengpei{Using QP to solve for combinatorics is not actually quite common. References: }

\item \fengpei{possibly directly usable results: \cite{chaovalitwongse2004new,sherali2007improved}, maybe will write a section later}
\end{itemize}


 
\section{possible LP relaxation of the QP}
This paper \cite{kimizuka2019solving} claims that if in the QP, $Q$ has zero diagonal then there is an LP relaxation for it where the solution to the LP is equal to the solution to the QP. Though this stackexchange persoon has problems with it https://or.stackexchange.com/questions/5824/is-this-semidefinite-constraint-in-fact-pointless


CPLEX OPTIMAL: https://or.stackexchange.com/questions/503/cplex-non-convex-quadratic-programming-algorithms


\subsection{ A mixed integer LP}
A mixed integer may be slightly easier? 


\subsection{Semi-definite Programming }

Using SDP to relax combinatorics problems turn out to be quite common (numerous reference exists here, none of which directly applies here, most famous example is MAXCUT, with 0.89 ratio of duality gap). 

\arash{ Yes, but usually they have the same power as LP. Explain how does it avoid the bad configurations and how do you round the SDP?  }  

\fengpei{Not sure whether they have same power as LP. Yeah I also have no good way to round it for a $k$-cluster case when $k>2$... I wrote another Mixed-integer LP formulation. It may be helpful}

\arash{Does the SDP imply the LP1 when there is no $\#$ of moves constraint? If so, then we should mention that we can round the SDP similar to the ones used for LP2.}



They usually provide good relaxtion (sometimes exact, no duality gap), and it is a fairly standard tool for these situations. They are also convex and can be solved very efficiently by off-the-shelf solvers. 

Let's first consider the following formulation.


\begin{table}[hht]
    \centering
    \begin{tabular}{lllr}
    \toprule
        \texttt{Minimize:} & $x^TCx$ & &\\
        \texttt{Subject to:} & & &\\
        & $Ax=e$,  & (S1)\\
        & $a^Tx\leq M$ & (S2)\\
        & $x_i(1-x_i)=0$ for all $i$ & (S3)\\
        \bottomrule
    \end{tabular}
    \caption{Quadratic objective with Quadratic constriant}
    \label{tab:my_labelqpqp}
\end{table}





In our specific problem, we have $x\in \mathbb R^{|V|k}$, let $x^n_i$ ($n\in[|V|], i\in[k]$) represents the "presence" or (weight) of the $n$-th node on cluster $i$, $x$ would look like 
\begin{equation*}
    x^T=[x^1_1,x^1_2,x^1_3,...,x^1_k, x^2_1,x^2_2,...x^2_k,...,x^{|V|}_{k-1},x^{|V|}_k]
\end{equation*}
Our $C\in\mathbb R ^{|V|k\times|V|k}$ would satisfy $C_{x^n_ix^m_j}=c_{uv}$ where $u$ is the $n$-th node and $v$ is the $m$-th node. (Note $c_{uu}=0$). Next we have $A\in\mathbb R ^{|V|\times|V|k}$ with the $n$-th row $a^T_n$ ($n\in[|V|]$) having entries 1 in the $k$ positions corresponding to $x^n_1,x^n_2,...x^n_k$ and 0 otherwise. Then $e\in\mathbb R^{|V|}$ represents the vector of one's. Then $a^T$ is the vector that sums up the entries of the node in all $k$ position excluding the previous location. Basically, for entries of $a$, in the entry corresponding to $x^n_i$, if the $n$-th node is already at cluster $i$, then this entry of $a$ is 0 and 1 otherwise. $M$ is the movement budget (an integer). Finally, note (S3) is actually a quadratic constraint: Let $e^i$ denote the standard vector in the $i$-th direction ($e^i$ is a vector that equals 1 in the $i$-th position and 0 otherwise), let $D_i=\text{diag}(e_i)$ be the matrix with elements of $v$ as diagonal, then 
\begin{equation*}
    x_i(1-x_i)=0\text{ for all } i \iff x^TD_ix-e_i^Tx=\boldsymbol{0}
\end{equation*}

Note we are writing $x$ in the general formulation, not the "node then cluster" specifics. Do not get confused...

\textbf{Remark} Note here $C$ is not positive semi-definite (or negative definite). I note here the constraint (S3), which is the integer constriant in quadratic form, is actually important in the formulation of SDP, otherwise the SDP relaxtion would not be feasible. Even though we already know with our case (using the proof before), we know the solution has integer form and (S4) is indeed redundant (for this specific problem, we are adding the (S4) constraint which is already satisfied by the optimal solution, which has no effect on the optimal value ). But in general, we do need (S3) for this SDP relaxtion to work.
\subsection{formulation 1}
The next two SDP formulation are dual of each other (equivalent), they are the same relaxation (lower bound) of the original problem. Which one works better needs to be seen. We first present 1
\begin{table}[hht]
    \centering
    \begin{tabular}{lllr}
    \toprule
        \texttt{Maximize:} & $\theta$ & &\\
        \texttt{Subject to:} & & &\\
        & $\begin{pmatrix} \lambda^Te-\xi\cdot M-\theta & \frac{1}{2}(\xi\cdot a^T-\lambda^TA-\rho^T)\\ \frac{1}{2}(\xi\cdot a^T-A^T\lambda-\rho) & C+\text{diag}(\rho) \end{pmatrix}\succcurlyeq 0,$  & (S1)\\
        & $\xi\geq 0$ & (S2)\\
        \bottomrule
    \end{tabular}
    \caption{SDP 1}
    \label{tab:my_label}
\end{table}
Here $\xi$ has dimension 1, the rest (vectors $\lambda$ and $\rho$) can be figured out by matching dimensions of $A$ from (S1). The next formulation is the dual of the above one, which might be more intuitive to understand.

\subsection{formulation 2}

Let $\bar C=\begin{pmatrix} 0 & 0\\ 0 & C\end{pmatrix}$, $\bar E_i=\begin{pmatrix} 0 &-\frac{1}{2}e_i^T\\ -\frac{1}{2}e_i & \text{diag}(e_i)\end{pmatrix}$, $\bar A_n=\begin{pmatrix} -1 &\frac{1}{2}a_n^T\\ \frac{1}{2}a_n & 0\end{pmatrix}$ where $a_n^T$ is the $n$-th row of $A$. Finally, let $\bar A = \begin{pmatrix} 0 &\frac{1}{2}a^T\\ \frac{1}{2}a & 0\end{pmatrix} $ be from (S2). The other formulation is (notice now we assume $X\in\mathbb R^{(|V|k+1)\times (|V|k+1)}$)

\begin{table}[hht]
    \centering
    \begin{tabular}{lllr}
    \toprule
        \texttt{Minimize:} & $Tr(\bar C X)$ & &\\
        \texttt{Subject to:} & & &\\
        & $Tr(\bar E_i X)=0$ \text{for all $i\in[|V|k]$} & (S1)\\
        & $Tr(\bar A_n X)=0$ \text{for all $n\in[|V|]$} & (S2)\\
        & $Tr(\bar A X)\leq M$  & (S3)\\
         & $X_{11}=1$ & (S4)\\
          & $X\succcurlyeq0$  & (S5)\\
        \bottomrule
    \end{tabular}
    \caption{SDP 2}
    \label{tab:my_label}
\end{table}
The formulation is basically equivalent to \ref{tab:my_labelqpqp}, except we dropped a rank-one constraint (i.e., $\text{rank}(X)=1$. Indeed we did not write out $X=\begin{pmatrix} 1\\ x \end{pmatrix}\begin{pmatrix} 1\\ x \end{pmatrix}^T$ basically), because this is not a convex constraint).

\subsection{ A mixed integer LP}
A mixed integer may be slightly easier? or maybe it will help to Now we write 
\begin{table}[hht]
    \centering
    \begin{tabular}{lllr}
    \toprule
        \texttt{Minimize:} & $x^TCx$ & &\\
        \texttt{Subject to:} & & &\\
        & $Ax=e$,  & (S1)\\
        & $a^Tx\leq M$ & (S2)\\
        & $x_i\in\{0,1\}$ for all $i$ & (S3)\\
        \bottomrule
    \end{tabular}
    \caption{Quadratic objective with mixed integer}
    \label{tab:my_labelqpmi}
\end{table}

Because the weight of $C$ is non-negative and square in shape, we can show it is equivalent to (\cite{chaovalitwongse2004new}) 
\begin{table}[htt]
    \centering
    \begin{tabular}{lllr}
    \toprule
        \texttt{Minimize:} & $e^Tz$ & &\\
        \texttt{Subject to:} & & &\\
        & $Ax=e$,  & (L1)\\
        & $a^Tx\leq M$ & (L2)\\
        & $Cx-y-z=0$,  & (L3)\\
        & $y^Tx=0$,  & (L4)\\
        & $x_i\in\{0,1\}$ for all $i$ & (L5)\\
        & $y,z\geq \boldsymbol{0}$,  & (L6)\\
        \bottomrule
    \end{tabular}
    \caption{linear with mixed integer}
    \label{tab:my_labelblmi}
\end{table}

which is also equivalent to the following (let $M_C$ be a constant where $M_C\geq \max_i\sum_j|C_{ij}|$)

\begin{table}[htt]
    \centering
    \begin{tabular}{lllr}
    \toprule
        \texttt{Minimize:} & $e^Tz$ & &\\
        \texttt{Subject to:} & & &\\
        & $Ax=e$,  & (L1)\\
        & $a^Tx\leq M$ & (L2)\\
        & $Cx-y-z=0$,  & (L3)\\
        & $y\leq M_C(e-x)$,  & (L4)\\
        & $x_i\in\{0,1\}$ for all $i$ & (L5)\\
        & $y,z\geq \boldsymbol{0}$,  & (L6)\\
        \bottomrule
    \end{tabular}
    \caption{linear with mixed integer}
    \label{tab:my_labelblmi}
\end{table}

\fengpei{What if we round the LP (or some other intelligent initial solution) and use it as a starting point for these Mixed-integer LP formulation? Smart things has to be done here cuz the size is still too big for integer programming. }

\newpage
\subsection{Observation}

The optimization in table \ref{tab:my_labelqpqp} would maintain the same optimal solution if we add change $C$ to $C-\lambda I$ for any $\lambda$. To see this, simply note the fact that the objective value decrease by $\lambda|V|$ for any feasible solution regardless. Thus, if $\lambda\geq \lambda_{\text{max}}(C)$, then $C-\lambda I$ becomes negative semi-definite. Minimization of negative semi-definite quadratic form is NP-hard, but may have bound on SDP duality gap (MAXCUT is maximizing positive definite matrix, it has bound on how good is the SDP gap). Thus, we may deduce bound based on eigenvalue of $C$.

%\fi 


\section{Notes on Experiments}
MS division GBR IND CAN graph would give fractional solution with the LPs but gives int solution with QP.

So far quite fast, even faster than the LP. Though haven't extensively tested. on a 3600 node graph, with max move = 7, took 1.5 min. on 16k node graph with max move = 10 in 17 mins!

Also the biggest graph we have is not 60k, it is around 20k, because we compress business nodes.

%\mina{how are we gonna round it? I think it would give integer solutions most of the time for the MS specific graphs: if let's say the fractional solution says take $v$ with 0.5 probability to $i$ and take $u$ with 0.5 probability to $j$, then the cut reduction from taking $u$ to $j$ is exactly the same as cut reduction from taking $v$ to $i$. So the communications of two nodes are basically the same which doesn't happen often. Also to avoid this, we can perturb the edge weights a bit!}

%\mina{Also if the solution says $X_v^i=p_1$ and $X_v^j=p_2$}




==> wrong_lin_alg.tex <==

\subsection{$O(M)$-approximation algorithm \mina{Not correct!}}
%\mina{we can reduce the problem to the following: suppose the initial partitioning has all nodes in cluster 1 (except for terminal). what is the best clustering so that at most M nodes leave cluster 1?}

\begin{theorem}
Let $M$ be any positive real number. There is a $8M$- approximation algorithm for max-$M$-move $k$-partitioning in $k^{O(M^2)}T(n)$ time, where $T(n)$ is the running time of solving a linear program with $O(n)$ variables and $O(n)$ constraints. 
\end{theorem}

\begin{algorithm}[h]
\caption{Base cases}\label{alg:basecases}
\begin{algorithmic}[1]
    \State Let $A$ be all the nodes $v$ with $X_v^{\ell_v}\ge 3/4$ and $A'=V(G)\setminus A$.
    \If{$M<2$}
        \State compute the cut achieved by moving a node $v$ to any of the clusters $1,\ldots,k$.
        \State \Return The smallest cut computed.
    \ElsIf{$n<6M$}
        \State compute all cuts achieved by moving at most $M$ nodes. 
         \State \Return The smallest cut computed.
    \Else 
    \State \Return Not a base case.
    \EndIf
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[h]
\caption{$8M$-approximation algorithm for max-$M$-move $k$-cut \mina{indent cases}}\label{alg:8M_algorithm}
\begin{algorithmic}[1]
    \Require{Input graph $G$, parameter $M$}
    \State run Base Case Algorithm \ref{alg:basecases}.
    \State $X\gets$ solution to the LP of Table \ref{tab:maxmove-lp}. 
    \If{$G,M$ is a base case}
        \State \Return the output of Algorithm \ref{alg:basecases}.
    \EndIf
    \State $A\gets$ any $v\in V(G)$ with $X_v^{\ell_v}\ge 3/4$.
    \State $A'\gets V(G)\setminus A$
    \State Create the graph $G'$: $V(G'):=V(G)$ and $uv\in E(G')$ if $uv\in E(G)$ and $d_X(u,v)<g=\frac{1}{8M}$.
    

    \State We have the following cases:
    \State \textbf{Case 1.} $G'$ has more than one connected component
    \For{each connected component $H$ of $G'$}
            \State Recurse on $H$ with move parameter $\sum_{v\in H}(1-X_v^{\ell_v})$, let $Z_H$ be the recursion solution.
            \State \Return $Z = \cup_H Z_H$.
        \EndFor
    
    \State Let $i^*$ be the cluster where for all $v\in A$, $\ell_v=i^*$ \Comment{such cluster exists when $G'$ has one connected component}
    \State \textbf{Case 2.} $G'$ has one connected component and for all $v\in A'$, $\ell_v=i^*$. 
            \State \Return the solution $Z$ where $Z_v=e_{i^*}$ for all non-terminal nodes $v$.
    \State \textbf{Case 3.} $G'$ has one connected component and $|A'|\le M$
    %\State Let $i^*$ be the cluster such that for all non-terminal $v\in A$, $\ell_v=i^*$.
        \State \Return $Z$ where for all $v\in G$, $Z_v=e_{i^*}$.
    \State \textbf{Case 4.} $G'$ has one connected component and $|A'|\ge \floor{M}+1$
        \For{All assignments $Y_v$ of vertices of $A'$ to the $k$ partitions $\{e_1,\ldots,e_k\}$ such that $\sum_{v\in A'}Y_v^{\ell_v}\ge |A'|-M$}
            \For{All $i\in \{1,\ldots,k\}$}
            \State $A_i'\gets $ all nodes $v\in A'$ that are assigned to cluster $i$, i.e. $Y_v=e_i$.
            \EndFor
        \State $M'\gets \sum_{v\in A'}(1-Y_v^{\ell_v})$ is the number of nodes in $A'$ that are moved.
        \State Create the graph $H^{(Y)}$ by contracting each set $A_i'\cup \{s_i\}$ into a new node $s_i^*$
        \State Let $Z^{(Y)}$ be the solution to the recursion on $H^{(Y)}$ with the move parameter $M-M'$. Extend $Z^{(Y)}$ from $H^{(Y)}$ to $G$ below.
        \For{All $i\in \{1,\ldots,k\}$}
            \For{All $v\in A_i\cup s_i$}
            \State define $Z^{(Y)}_v=e_i$
            \EndFor
        \EndFor
        \EndFor
    \State \Return $Z^{(Y)}$ that minimizes the cut over all $Y$.
    
\end{algorithmic}
\end{algorithm}






\begin{proof}
We first describe our algorithm along with intuitions for different steps, and then prove the approximation guarantees of it. The base cases of our algorithm is depicted in Algorithm \ref{alg:basecases} and the main algorithm is in Algorithm \ref{alg:8M_algorithm}.

First we consider that $M\ge 2$. Otherwise for each non-terminal node $v$ and each cluster $i$, compute the cut obtained by moving $v$ to cluster $i$. Among all these cuts and the initial cut, output the one that is smallest. This is the first case in Algorithm \ref{alg:basecases}.

So from here we assume that $M\ge 2$.
Consider a solution $X$ of the max-$M$-move $k$-partitioning linear program. Let $A$ be the set of nodes $v$ such that $X_v^{\ell_v}\ge 3/4$. Let $A'$ be the rest of the nodes. By Lemma \ref{lem:size}, we have that $|A'|< 4M$.

We create a graph $G'$ with the same vertices as $G$ as follows. Let $g=\frac{1}{8M}$ be a gap parameter. For every $u$ and $v$, attach $u$ and $v$ in $G'$ if they are attached in $G$ and $d_{X}(u,v):=\frac{1}{2}\sum_i |X_u^i-X_v^i|< g$. From here we have three cases.
\begin{itemize}
    \item \textbf{Case 1.} Suppose $G'$ has more than one connected component. Then we recurse on each component $H$ with move parameter $M_H:=\sum_{v\in H}(1-X_v^{\ell_v})$. The base case of this recursion is when $H<6M$. The output solution is  the union of the solutions of each component.
    
    If $G'$ is connected, by Lemma \ref{lem:connected-comp}, for every $u,v\in A$, if $\ell_u\neq \ell_v$ then $u$ and $v$ are in different connected components in $G'$. So there is a $i^*$ such that for all $v\in A$, $\ell_v=i^*$.
    \item \textbf{Case 2.} Suppose that $G'$ is connected and for all $v\in A'$, $\ell_v=i^*$. In this case we don't move any nodes, so the solution $Z$ that the algorithm outputs is $Z_v=e_{i^*}$ for all non-terminal nodes $v$.
    \item \textbf{Case 3.} Suppose that $G'$ is connected and $|G'\setminus A|=|A'|\le M$. In this case we move all non-terminal nodes to $i^*$.
    \item \textbf{Case 4.} Suppose that $G'$ is connected and $|A'|\ge \floor{M}+1$. Consider all assignments of nodes in $A'$ to the $k$ clusters such that at most $M$ of them move from their primary cluster. There are at most $k^{|A'|}<k^{4M}$ such assignments. For each assignment, we are going to decide how to move the remainder of the nodes which are the nodes in $A$ recursively as follows. Consider an assignment $Y$ of nodes in $A'$, and suppose that $M'\le M$ nodes have been moved. 
    For each $i$ let $A_i'$ be the nodes in $A'$ that are assigned to cluster $i$. ``Contract" all these nodes with $s_i$, the terminal in cluster $i$, and call this ``super-node" $s_i^*$. For each node $u\notin A_i'$ define the $s_i^*u$ weight $c_{s_i^*u}=\sum_{v\in A_i'\cup \{s_i\}}c_{vu}$. Let the resulting graph be $H^{(Y)}$ with terminals $s_1^*,\ldots, s_k^*$ and with move parameter $M-M'$. 
Since $|A'|>1$, the number of nodes in $H$ is less than $G$, and we can recurse on $H$. 

The base of the recursion consists of three cases. The first two cases are when $M<2$ and when $n<6M$ which are described above. The third case is when all nodes $v\in A'$ also have $\ell_v=i^*$. For this special case of input, we don't recurse on the configuration where none of the nodes in $v$ move. Formally, consider the configuration $Y$ where for all nodes $v\in A'$ we have $Y_v=e_{\ell_v}$. We won't recurse on $H^{(Y)}$. Instead, we output the solution where we move no nodes. All the other base cases are depicted in Algorithm \ref{alg:basecases}.

We then output the solution with the least cut among all the configurations as the final solution of our algorithm. Note that for any configuration that we recurse on, if $Z$ is the solution this instance, then for any $u$ that is contracted into $s_i^*$ we let $Z_u=Z_{s_i^*}$.
\end{itemize}
The approximation factor is proved to be $8M$ in Lemma \ref{lem:approx-guarantee}
 and the running time of the algorithm is proved in Lemma \ref{lem:runningtime}.
%Now the running time of this case is at most $k^{4M}F(n-1)$. The running time of the algorithm is dominated by this step, and so we have $F(n)\le T(n)+k^{4M}F(n-1)$ \mina{not complete}
\end{proof}

\begin{lemma}\label{lem:approx-guarantee}
Algorithm \ref{alg:8M_algorithm} is a $8M$-approximation algorithm for max-$M$-move $k$-partitioning.
\end{lemma}
\begin{proof}\mina{change the Y in prelim.}
Let $Z$ be the solution of our algorithm and let $\bar{Z}$ be the optimal integer solution. Let $X$ be the optimal LP relaxation solution of the \maxmove instance. \mina{fix this} If $G'$ is not connected (Case 1), then for each connected component $H$ we have $\sum_{vu\in E(H)} c_{uv}d_Z(u,v)\le \frac{1}{g}\sum_{vu\in E(H)} c_{uv}d_{\bar{Z}}(u,v)$. This is because if $X'$ is an LP solution for $H$, then $\sum_{vu\in E(H)} c_{uv}d_X(u,v)\ge \sum_{vu\in E(H)} c_{uv}d_{X'}(u,v)$, and from recursion assumption we have that $\sum_{vu\in E(H)} c_{uv}d_Z(u,v)\le \frac{1}{g}\sum_{vu\in E(H)} c_{uv}d_{X'}(u,v)$. Now for each $u$ and $v$ that are not in the same connected component we have that $d_X(u,v)>g$, so $d_Z(u,v)\le \frac{1}{g}d_X(u,v)$. So the cut value created by $Z$ is at most $\frac{1}{g}=8M$ times the value of the cut created by the LP solution. Note that the max move condition is equivalent to $\sum_v (1-X_v^{\ell_v})\le M$, so we have $\sum_H M_H\le M$ and we have moved at most $M$ nodes.

So suppose that $G'$ is connected. In this case by Lemma \ref{lem:connected-comp} there is a node $i^*$ such that for all non-terminal nodes $v\in A$, $\ell_v=i^*$ \mina{make sure you always say non-terminal}. First suppose that for all $v\in A'$, $\ell_v=i^*$ (Case 2). In this case the solution of the algorithm is $Z_v=e_{i^*}$ for all non-terminal nodes $v$. Any cut in this solution is of the form $us_i$ where $i\neq i^*$. Now since $|A'|<4M$, any node $u$ is either in $A$ or is at most $4M$ edges away from $A$ in $G'$. If $v$ is the closest node in $A$ to $u$, then we have $d_X(u,v)\le 4gM<1/2$, so $|X_u^{i^*}-X_v^{i^*}|\le 1/2$. Thus we have $X_u^{i^*}\ge 1/4$. So $d_X(u,s_i)\ge |X_u^{i^*}-X_{s_i}^{i^*}|\ge 1/4$, and we have $d_Z(u,s_i)\le 4d_X(u,s_i)$. So the cut that $Z$ creates has value at most four times the cut that the LP creates.

Now suppose that $|A'|\le M$ (Case 3). In this case the algorithm moves all the nodes in $A'$ to $i^*$, and so any edge in the cut is of the form $us_i$ for $i\neq i^*$. For any non-terminal $u$, either $u$ is in $A$ or is connected to a node in $A$ with a path of length at most $M$. So $X_u^{i^*}\ge 3/4-Mg>1/2$. 
Since $X_{s_i}=e_i$, $d_X(u,s_i)\ge 1/2$ and so $d_Z(u,s_i)\le 2d_X(u,s_i)$. So the cut value created by $Z$ is at most twice the cut value that $X$ represents. So $Z$ is in fact a $2$-approximation. 

Finally suppose that $|A'|\ge \floor{M}+1$ (Case 4).
Let $\bar{Z}$ be the optimal integer solution to the problem. We have considered the case where we partition the nodes in $A'$ exactly like $\bar{Z}$. Let the graph resulting from the contractions be $H$. Note that if we contract nodes $u$ a $v$ into $s_i^*$ for some $i$, it must be that $\bar{Z}_v=\bar{Z}_u=i$. 
Recall that $A_i'$ is the set of all the nodes contracted into $s_i^*$. By defining $Y_{s_i^*}=e_i$ we see that the value of the cut that $Y$ represents in $G$ doesn't change in $H$, i.e. $\sum_{uv\in E(G)}c_{uv}d_{\bar{Z}}(u,v) = \sum_{uv\in E(H)}c_{uv}d_{\bar{Z}}(u,v)$. Let $\bar{Z}_H$ be the optimal integer solution for $H$. So we have $\sum_{uv\in E(H)}c_{uv}d_{\bar{Z}}(u,v)\ge \sum_{uv\in E(H)}c_{uv}d_{\bar{Z}_H}(u,v)$. Moreover, from recursion, if $Z$ is the solution that the algorithm outputs, we have $\frac{1}{g}\sum_{uv\in E(H)}c_{uv}d_{\bar{Z}_H}(u,v)\ge \sum_{uv\in E(H)}c_{uv}d_{Z}(u,v)$. So we have 
\begin{align*}
\frac{1}{g}\sum_{uv\in E(G)}c_{uv}d_{\bar{Z}}(u,v) = 
    \frac{1}{g}\sum_{uv\in E(H)}c_{uv}d_{\bar{Z}}(u,v)\ge \sum_{uv\in E(H)}c_{uv}d_{Z}(u,v) = \sum_{uv\in E(G)}c_{uv}d_{Z}(u,v)
\end{align*}
Note that for the last equality we used the fact that for all the nodes $u$ contracted into $s_i^*$, we let $Z_u=Z_{s_i^*}$. So $Z$ is a $\frac{1}{g}$-approximation. 
\end{proof}
\begin{lemma}\label{lem:runningtime}
Algorithm \ref{alg:8M_algorithm} runs in time $k^{O(M^2)}T(n)$ where $T(n)$ is the running time of solving a linear program with $O(n)$ variables and $O(n)$ constraints. 
\end{lemma}
\begin{proof}
Let $F(n,M)$ be the running time of Algorithm \ref{alg:8M_algorithm} on instances of \maxmove on instances with $n$ nodes. We show that $F(n,M)\le k^{O(M^2)}O(T(n))$, where $T(n)$ is the running time of solving a linear program with $O(n)$ variables and $O(n)$ constraints. We assume that if $n_1+n_2=n$, $T(n_1)+T(n_2)\le T(n)$, and that $T(n)\ge n$. 

In fact we prove that $F(n,M)\le 2k^{4M(M-1)}T(n)$.
First consider the special instances where there is $i^*$ such that for all non terminal nodes $v$ we have $\ell_v=i^*$. Let the running time of this case be denoted by $F'(n,M)$. First note that any instances produced in the algorithm to recurse on is of this type. To see this, observe that the recursions only happen on case 1 and case 4. In case 1, each connected component of $G'$ will also have all non-terminal nodes initially belonging to $i^*$. and in case 4, in any assignments of nodes in $A'$ to clusters, all the nodes that haven't been contracted are a subset of non-terminal nodes in $G$ so they all  non-terminal nodes in those graphs also initially belong to $i^*$.

We show that $F'(n,M)\le T(n)k^{2M(M-1)}-2$, and to do that we recurse on $M$.

For case 1 of the algorithm we have that $F'(n,M)\le \sum_H F'(|H|,M_H)$ where the sum is on the connected components $H$ of $G'$, and we have $\sum_H |H|=n$ and $\sum_H M_H\le M$. Since $T(n)\ge \sum_H T(n_H)$ and $m_H\le M$ for all $H$, we have $F'(n,M)\le T(n)k^{2M(M-1)}-2$. 

Case 2 and 3 have linear running times. So suppose that we are in case 4 of the algorithm. Recall that we consider all assignments of nodes in $A'$ to clusters $1,\ldots,k$ such that at most $M$ of them move from their original clusters. For the assignment where every node in $A'$ is assigned to its initial cluster, the recursion stops in case 2, since all nodes are from cluster $i^*$. 

For all the other assignments, at least one node in $A'$ is assigned to a cluster other than its initial cluster. Moreover the size of these graphs are at most $n-1$, since $A'>1$.
So we have $F'(n,M)\le k^{4M}+k^{4M}F'(n-1,M-1)$. The first term is due to the comparison of results at the end. We also assume that $O(n)\le k^{4M}F'(n-1,M-1)$, since the algorithm takes linear time to read the input. By our recursion on $M$, we have that $F'(n-1,M-1)\le k^{2(M-1)(M-2)}T(n-1)-2$. So we have $F'(n,M)\le k^{4M}+k^{2M(M-1)}T(n-1)-2k^{2M(M-1)}\le k^{2M(M-1)}T(n)-2$.% (we used the fact that $2k^{2M(M-1)}-k^{4M}\ge 2$.

%(say we use the fact that $F(n,M)\ge F(n',M')$ for $n\ge n'$ and $M\ge M'$).
Now to prove the bound on $F$, we use a similar approach. We use a recursion on $M$. Cases 1,2 and 3 are the same as above. To analyze case 4, first consider the assignment that assigns all nodes in $A'$ to their initial partition. The graph resulting from contracting nodes in this case has all non-terminal nodes belonging to a cluster $i^*$, and so the running time is at most $F'(n-1,M)$. For all the other assignments, we have at least one node in $A'$ that is assigned to a partition other than its initial partition, and so the max move parameter of the resulting graph is at most $M-1$.

So we have that $F(n,M)\le F'(n-1,M)+ k^{4M}F(n-1,M-1)\le k^{2M(M-1)}T(n)+k^{4M}F(n-1,M-1)$. Using recursion assumption on $M$, we have that $F(n-1,M-1)\le 2k^{4(M-1)(M-2)}T(n-1)\le 2k^{4(M-1)(M-2)}T(n)$, and so $F(n,M)\le T(n)(2k^{4(M-1)(M-2)}+k^{2M(M-1)})\le 2k^{4M(M-1)}T(n)$. 
\end{proof}

